Generalised Quantum Enveloping Algebras, Coloured Kac-Moody Algebras, and Langlands Interpolation

We propose in this thesis a new deformation process of Kac-Moody algebras and their representations. The direction of deformation is given by a collection of numbers, called a colouring. The natural numbers lead for example to the classical algebras, while the quantum numbers lead to the associated quantum algebras. We first establish sufficient and necessary conditions on colourings to allow the process depend polynomially on a formal parameter and to provide the generalised quantum enveloping (GQE) algebras. We then lift the restrictions and show that the process still exists via the coloured Kac Moody algebras. We formulate the GQE conjecture which predicts that every representation in the category Oint of a Kac-Moody algebra can be deformed into a representation of an associated GQE algebra. We give various evidences for this conjecture and make a first step towards its resolution by proving that Kac-Moody algebras without Serre relations can be deformed into GQE algebras without Serre relations. In case the conjecture holds, we establish an analog result for coloured Kac-Moody algebras, we prove that the deformed representation theories are parallel to the classical one, we explicit a deformed Serre presentation for GQE algebras, we prove that the latter are the representatives of a natural class of formal deformations of Kac-Moody algebras and are h-trivial in finite type. As an application, we explain in terms of interpolation both classical and quantum Langlands dualities between representations of Lie algebras, and we propose a new approach which aims at proving a conjecture of Frenkel-Hernandez. In general, we prove that representations of two isogenic coloured Kac-Moody algebras can be interpolated by representations of a third one. Observing that standard quantum algebras satisfy the GQE conjecture, we give a new proof of the previously mentioned classical Langlands duality.

==> Cohomology/main_coho.tex <==
\setcounter{section}{0}
\setcounter{equation}{0}
\setcounter{thm}{0}
\setcounter{introthm}{0}
\setcounter{introconj}{0}

\selectlanguage{english}



\begin{abstract}
We relate the cohomology theory of a Kac-Moody algebra to the cohomology theory of the associated Lie algebra without Serre relation. We obtain results about the latter. In particular, the free Serre relations version of second Whitehead's lemma is established. This last result was the original motivation of this paper and is used in part \ref{part_GQE} to define the generalised quantum enveloping algebras. In part \ref{part_BKM} these algebras are applied in order to solve conjectures of Frenkel and Hernandez (see \cite{FH}) and to give new results, about Langlands interpolating quantum algebras.
\end{abstract}





\section{Introduction}
Among all the subjects where cohomology of Lie algebras  enters the game, one can cite (formal) deformation theory. Indeed, Hochschild cohomology of an universal enveloping algebra can be related to the cohomology of the associated Lie algebra and in another hand Hochschild cohomology controls the ways various algebraic structures can be deformed (see \cite{Ger}). \\

Let $\glie$ be a semisimple finite-dimensional Lie algebra (over a field of characteristic 0). First and second Whitehead's lemmas assert that the cohomology of  $\glie$ with coefficients in any finite-dimensional $\glie$-module vanishes, in degree 1 and in degree 2 respectively. \\

Second Whitehead's lemma implies (see for example \cite[th\'eor\`eme 2.5.5]{Gui} or \cite[theorem XVIII.2.2 and corollary XVIII.3.3]{Kas}) that there is only one possible formal deformation, namely the trivial one, of the associative algebra $U(\glie)$. In a deformation sense, $U(\glie$) is rigid. As for first Whitehead's lemma, it implies (see for example \cite[th\'eor\`emes 2.5.6 \& 2.5.7]{Gui}) that finite-dimensional $\glie$-modules cannot be deformed in a non trivial way. \\

Previous rigidity results have then important direct consequences in quantum groups theory. Denote by $U_h(\glie)$ the quantum group associated to $\glie$. It is a (topological) Hopf algebra, which deforms the enveloping algebra $U(\glie)$, considered with its natural Hopf algebra structure. $U_h(\glie)$, as an associative algebra, is thus merely the same object than $U(\glie)$ and representation theory of $U_h(\glie)$ is parallel to $\glie$'s one. Note however that, seen as a Hopf algebra, the quantum group $U_h(\glie)$ is a non trivial deformation of $U(\glie)$.



\subsection*{Questions}

Denote by $\tglie$ the Lie algebra defined by the same generators and relations than $\glie$, but where Serre relations are omitted. There exist some connections between representation theories of the two Lie algebras $\glie$ and $\tglie$. First, one can make the following straightforward remark: since $\glie$ is a quotient of $\tglie$, a $\glie$-module is by restriction a $\tglie$-module. Conversely, it is known that Serre relations are satisfied in all finite-dimensional $\tglie$-modules (see \ref{para_gtildeg}), in other words a finite-dimensional $\tglie$-module is in fact the restriction of a $\glie$-module. Moreover, one can define the category $\tilde {\mathcal O}$ for $\tglie$ in a similar way than the category ${\mathcal O}$ for $\glie$ (see \ref{para_Ocat} for definitions). It appears that a simple $\tglie$-module in $\tilde {\mathcal O}$ is actually the restriction of a simple $\glie$-module in ${\mathcal O}$ (see again \ref{para_gtildeg}). \\

One can ask the following questions.

\begin{quest} \label{quest_reprtgrigid}
Is finite-dimensional representation theory of $\tglie$ still rigid?
\end{quest}

\begin{quest} \label{quest_utgrigid}
Is the associative algebra $U(\tglie)$ still rigid?
\end{quest}

We have previously evoked that Whitehead's lemmas provide answers to these questions in the case of $\glie$. Thus one is naturally leaded in asking the two following questions.

\begin{quest} \label{quest_fsrwhitehead1}
Is there an analog (which we will call the free Serre relations version) of first Whitehead's lemma when one consider $\tglie$ instead of $\glie$? \\
In other words, does $\text H^{\, 1}(\tglie,M)$ vanish for all finite-dimensional $\tglie$-modules $M$?
\end{quest}

\begin{quest} \label{quest_fsrwhitehead2}
Is there an analog (which we will call the free Serre relations version) of second Whitehead's lemma when one consider $\tglie$ instead of $\glie$? \\
In other words, does $\text H^{\, 2}(\tglie,M)$ vanish for all finite-dimensional $\tglie$-modules $M$?
\end{quest}

Remark from now on that question \ref{quest_fsrwhitehead1} has a positive answer. The proof is quite straightforward, see remark \ref{rem_fsrvwl1}. As a consequence, in a same way than first Whitehead's lemma implies that representation theory of $\glie$ is rigid, its free Serre relations version gives a positive answer to question \ref{quest_reprtgrigid}.



\subsection*{Motivations}
Let us briefly expose the context these questions arised from. \\

Frenkel and Hernandez defined what they called Langlands Interpolating Quantum (LIQ) groups: see \cite{FH}. The LIQ group associated to $\glie$ is an associative algebra related to the universal enveloping algebra $U(\tglie$). More precisely, this LIQ group provides some interpolation between the quantum group (without Serre relations) $U_q(\tglie)$ and its Langlands dual $U_t \! \left( \widetilde{{}^L \glie} \right)$ (the Langlands dual Lie algebra ${}^L \glie$ is defined as the semisimple Lie algebra whose Cartan matrix is the transpose of $\glie$'s one). \\

The representation theory of LIQ groups and its interpolation properties, motivated by geometric Langlands correspondence, remained until now conjectural. Other questions, for example the existence of Serre type relations in LIQ groups, were also left unanswered. For details about geometric Langlands program motivations, see the introduction of \cite{FH}. \\

In a recent work (see \cite{Bou1}), the author started to develop a new theory of LIQ algebras, in order to give a more precise sense to deformation properties and simplify interpolation properties of LIQ algebras. Nevertheless the main goal was to make possible the use of formal deformation theory. Like in the case of quantum groups, the hope was to apply rigidity results to LIQ algebras study. \\

The definition of rank 1 LIQ algebras, given in \cite{Bou1}, could be naturally extended to any rank but the LIQ algebra associated to $\glie$ would then be only a deformation of the universal enveloping algebra $U(\tglie)$. There was, at the time of this latter work, a priori no clue about how to deform Serre relations in a compatible way and even whether it was possible. The main conjecture made by Frenkel and Hernandez, transcribed in this new theory of LIQ algebras, involves representation theory of the latter. Again, there was a priori no clue about what the representation theory is. The two rigidity questions \ref{quest_reprtgrigid} and \ref{quest_utgrigid} then appear as natural (while seemingly too ambitious in the case of \ref{quest_utgrigid}) in an attempt to make significant advances in the investigation of representation theory and algebraic structure of LIQ algebras. \\

At this point it is worthwhile to note that LIQ algebras can be handled in the much larger framework of Generalised Quantized Enveloping (GQE) algebras (see part \ref{part_GQE}), where in particular previous investigations are naturally settled. GQE algebras are a general deformation theory of $U(\glie)$, expressed only from deformation data of the natural numbers. Note that quantum groups are GQE algebras by considering the quantum numbers as a deformation datum of the natural numbers. Others particular choices of deformation data provide new LIQ algebras, which generalise in a natural way LIQ algebras of rank 1 introduced in \cite{Bou1}. \\

In this article we give a positive answer to question \ref{quest_fsrwhitehead2}. In a same way than second Whitehead's lemma implies rigidity of $U(\glie)$, its free Serre relations version implies another rigidity result, closely related to question \ref{quest_utgrigid}. \\

It appears the Serre relations deformation problem in GQE algebras can be solved in an abstract way thanks to the free Serre relations version of second Whitehead's lemmas: see part \ref{part_GQE}. Representation theory of GQE algebras is then, as a consequence, proven to be parallel to $\glie$'s one. Conjectures of Frenkel and Hernandez and other properties of LIQ algebras are then derived in part \ref{part_BKM}. In the construction of GQE and LIQ algebras theories, this paper then provides a key technical ingredient. \\

Remark that, independently of their use in LIQ algebras theory, GQE algebras could be of great interest thanks to their natural and general definition. There exist some indications in this sense: see part \ref{part_GQE}.  \\

Kac-Moody algebras (see \cite{Kac} and \cite{Moo}) are infinite-dimensional Lie algebras, which provide a natural algebraic generalisation of semisimple finite-dimensional Lie algebras. Like in the case of the latter, one can associate to each Kac-Moody algebra $\glie$ a Lie algebra $\tglie$ defined by the same generators and relations than $\glie$, but where Serre relations are omitted. Remarks about some connections between the two representation theories remain valid (one has to substitute finite-dimensional modules with integrable modules in the general Kac-Moody case): see again \ref{para_gtildeg}. \\

As explained above, the main goal of this paper is to establish the free Serre relations version of second Whitehead's lemma. In the way chosen here of proving it, one is leaded in investigating connections between the cohomology theories of the semisimple finite-dimensional Lie algebras $\glie$ and $\tglie$. Most of the results and corollaries then obtained can be naturally generalised to the Kac-Moody general case. In another hand the author believes that GQE algebras theory can be extended to the Kac-Moody case (note the affine case is the next important aimed step in LIQ algebras theory, regarding geometric Langlands program motivations). For all these reasons, it has be chosen in this paper to work in the Kac-Moody general case.



\subsection*{Results}
Let us briefly describe the results proven in this paper and the ideas of their proofs. \\

Recall the original motivation of this paper was the free Serre relations version of second Whitehead's lemma: see theorem \ref{thm_swhlemma}. In the attempt to prove it, one is naturally tempted to adapt the proofs of usual second Whitehead's lemma. However several difficulties then appear. For example, the author does not know any analog of the Casimir central element in the Lie algebra without Serre relations $\tglie$ (in this discussion, $\glie$ is assumed to be finite-dimensional). In a same way, as far as the author knows, it could be difficult to describe the center of $U(\tglie)$ and no analog of the Harish-Chandra theorem currently exists. Another more modern approach can be envisaged, namely describe some blocks of the category $\widetilde {{\mathcal O}}$ of $\tglie$ (see \ref{para_Ocat} for the definition) and use related homological arguments, in a similar way than the one proposed by Kumar in \cite{KumBook}. Again, difficulties arise. \\

In this paper, we have chosen another way to prove theorem \ref{thm_swhlemma}. The idea is to use the usual second Whitehead's lemma to derive its free Serre relations version. We are then leaded in comparing, in a general manner, the cohomology theories of $\glie$ and $\tglie$. Fortunately, in degree 2, they will reveal themselves to be equal when the cohomology coefficients live in a finite-dimensional $\glie$-module (or equivalently in a finite-dimensional $\tglie$-module, as already mentioned). Actually, we are able to prove the equality of the two cohomologies, for more general cohomology coefficients $\glie$-modules. Besides, most of the results remain valid in the general case of (symmetrizable) Kac-Moody algebras. Let us now describe them. \\

We first, in proposition \ref{prop_ablie}, relate to each other the cohomologies of Lie algebras $\alie$ and $\blie = \alie / (\ilie \oplus \jlie)$, with coefficients in a $\blie$-module $M$. Assuming that cohomological dimensions of ideals $\ilie$ and $\jlie$ are strictly less than 2, we use two times Hochschild-Serre spectral sequences by considering successively the two quotients $\alie':= \alie / \ilie$ and $\blie \simeq \alie' / \jlie$. Thanks to the hypothesis on cohomological dimensions of $\ilie$ and $\jlie$, most of the terms in the second sheets of the two spectral sequences vanish. In another hand, since assuming the coefficients space $M$ is a $\blie$-module, the non zero terms in the spectral sequences involve trivial $\ilie$-modules and trivial $\jlie$-modules, which lead to easy computations of intermediate cohomologies. As a consequence, we are able to compare, in a quite simple and concrete way, the dimensions of the cohomologies of $\alie$ and $\blie$ with coefficients in the $\blie$-module $M$. Note that proposition \ref{prop_ablie} is the first of the two main technical pillar of this paper. \\

The situation of proposition \ref{prop_ablie} is a natural generalisation of the case we are interested in: $\blie$ is a Kac-Moody algebra $\glie$, $\alie$ is the associated Lie algebra without Serre relations $\tglie$, $\ilie$ and $\jlie$ are the ideals $\tslie^-$ and $\tslie^+$ of respectively negative and positive Serre relations (see \ref{para_slie}). The latter two ideals are Lie subalgebras of the two free Lie subalgebras of $\tglie$ respectively generated by negative and positive Chevalley generators. Thanks to a result of {\v{S}}ir{\v{s}}ov and Witt (see \cite{Shi} and \cite{Wit}), $\tslie^-$ and $\tslie^+$ are also free Lie algebras. It is besides known than the cohomological dimension of a free Lie algebra is stricly less than 2. The statement of proposition \ref{prop_ablie} then holds for the couple ($\tglie, \glie$): see theorem \ref{thm_htilde}. \\

In comparing the dimensions of the two cohomologies, the statement of theorem \ref{thm_htilde} involves the following $\glie$-modules, which we call the Serre modules: $S^-:= \tslie^- / [\tslie^-, \tslie^-]$, $S^+:= \tslie^+ / [\tslie^+, \tslie^+]$ (the $\glie$-module structure is described by the adjoint action: see the beginning of \ref{subs_ablie}) and $S = S^- \otimes_{\KK} S^+$. At degree $n$, the differences, between the two cohomologies of $\glie$ and $\tglie$ with coefficients in a $\glie$-module $M$, are quantified in terms of the Ext groups $\text{Ext}_{\glie}^m(S^{\pm},M)$ ($m = n-1,n-2$) and $\text{Ext}_{\glie}^m(S,M)$ ($m = n-2,n-3$). Keeping in mind that we originally wanted to establish the free Serre relations version of second Whitehead's lemma, we are thus leaded in proving vanishing of $\text{Ext}_{\glie}^0(S^{\pm},M)$, $\text{Ext}_{\glie}^1(S^{\pm},M)$ and $\text{Ext}_{\glie}^0(S,M)$. \\

The vanishing of $\text{Ext}_{\glie}^0(S,M)$, for all $\glie$-modules $M$ in the category ${\mathcal O}$, is the second technical pillar of this paper: see theorem \ref{thm_ext0S}. In order to manage it, we first start to study the Serre module $S^-$ and $S^+$. Thanks to the Cartan involution of $\tglie$, it appears that $S^+$ is the image of $S^-$ under the induced Cartan symmetry. We besides remark that $S^-$ is generated by the negative Serre relations (see lemma \ref{lem_negSerre}) and thus belongs to the principal block of the category $\Owg$ (see corollary \ref{cor_SOcat}). We then prove among others that $\text{Ext}_{\glie}^{\bullet}(S^{\pm},M)$ vanish when $M$ is outside the principal blocks of ${\mathcal O}$ and $\Owg$: see propositions \ref{prop_extneg} and \ref{prop_extpos}. Note however the last proposition holds only when $\glie$ is finite-dimensional, the general being only conjectured: see \ref{subs_further}. The vanishing of $\text{Ext}_{\glie}^0(S,M)$, for all $M$ in the category ${\mathcal O}$ is established in theorem \ref{thm_ext0S}. The proof is quite long and intermediate technical results are postponed in the appendix: see section \ref{sect_appendix}. An explanation of the ideas of the proof can be found in remark \ref{rem_ext0Sproof}. \\

The main results of this paper can now be easily derived.
\begin{enumerate}
\item[\textbullet] We prove the second cohomology group $\text H^2(\tglie)$ is isomorphic to the second cohomology group $\text H^2(\glie)$. See theorem \ref{thm_coho2}.
\item[\textbullet] Let $M$ be a $\glie$-module in ${\mathcal O}$, outside the principal blocks. It is known that $\text H^{\bullet}(\glie,M) = 0$. We prove that $\text H^1(\tglie,M)$ in the general case, and $\text H^2(\tglie,M)$ when $\glie$ is finite-dimensional, also vanish. When $\glie$ is infinite-dimensional, we prove that $\text H^2(\tglie,M)$ is isomorphic to $\text{Ext}^1_{\glie}(S^+,M)$. See theorems \ref{thm_h1kac}, \ref{thm_h2} and proposition \ref{prop_h2kac}. It is conjectured in \ref{subs_further} that the latter actually vanishes: see conjectures \ref{conj_extpos} and \ref{conj_h2kac}.
\item[\textbullet] We establish the originally wanted result of this paper, i.e. the free Serre relations version of second Whitehead's lemma: $\text H^2(\tglie,M) = 0$ for all finite-dimensional $\tglie$-modules, when $\glie$ is finite-dimensional. See theorem \ref{thm_swhlemma}. \\
As already said, the free Serre relations version of first Whitehead's lemma also holds and the proof is quite straightforward: see remark \ref{rem_fsrvwl1}.
\end{enumerate}

Note that all the results of this paper remain valid when one substitutes in their statements cohomology groups with homology groups and Ext groups with Tor groups. The proofs are similar or can be obtained by duality.



\subsection*{Organisation}
\begin{enumerate}
\item[\textbullet] In section \ref{sect_defi}, we recall some definitions and facts about characters (see \ref{subs_ch}), Kac-Moody algebras (see \ref{subs_kac}) and Yoneda extension groups (see \ref{subs_yoneda}).
\item[\textbullet] In section \ref{sect_ablie}, we investigate connections between the cohomology theories of two Lie algebras arranged in some special relative configuration (see \ref{subs_ablie}). We then apply the results to the case of a Kac-Moody algebra and of its associated Kac-Moody algebra without Serre relations (see \ref{subs_htilde}).
\item[\textbullet] In section \ref{sect_Serre}, we study the Serre modules $S^-$, $S^+$ and $S$. We first establish a Cartan symmetry between the negative Serre module $S^-$ and the positive one $S^+$ (see \ref{subs_SCartan}). We then study the negative Serre module (see \ref{subs_negSerre}). Finally (see \ref{subs_extvanish}) we prove in several cases the vanishing of some Serre Ext groups, among them: $\text{Ext}_{\glie}^0(S,M)$ for all $M$ in ${\mathcal O}$.
\item[\textbullet] In section \ref{sect_KWS}, we prove the main results of this paper, about cohomologies of a Kac-Moody algebra without Serre relations, namely: the second cohomology group (see \ref{subs_coho2}), the cohomology in degree 1 and 2 outside the principal blocks (see \ref{subs_principalblock}) and the free Serre relations version of second Whitehead's lemma (see \ref{subs_swhlemma}). In a last part (see \ref{subs_further}), we discuss about further directions.
\item[\textbullet] In section \ref{sect_appendix}, we collect several technical results, which are used in the different proofs of this paper. Note this appendix mainly serves theorem \ref{thm_ext0S}.
\end{enumerate}

For several reasons, already mentioned, one can be only interested in the free Serre relations version of second Whitehead's lemma. The results obtained in this paper are more general and, as a consequence, their proofs require more work than needed to only establish theorem \ref{thm_swhlemma}. Remarks, entitled ``Towards the free Serre relations version of second Whitehead's lemma" are present along all the way to the theorem. They indicate what can be skipped and how.



%\subsection*{Acknowledgments}
%This work is part of my PhD thesis. I would like to thank David Hernandez, my supervisor, for fiddly read-through and precious advices. Acknowledgements also goes to Dennis Gaitsgory for having granted me time, encouragements and remarks. I finally thank Dragos Fratila for interesting discussions about various topics related to this paper.





\section{Definitions} \label{sect_defi}
We recall some definitions and facts about characters, Kac-Moody algebras and Yoneda extension groups. \\

The part about characters is self-contained and all proofs are given. The goal is to give some basic results about generalised eigenspaces associated to characters. \\

About Kac-Moody algebras, only the facts needed in this part are recalled and most of the proofs are omitted. For details, the reader is referred to \cite{Kac} and \cite{KumBook}. The topics tackled are generalised Cartan matrices, the definition of Kac-Moody algebras, some basic results about their structures, the associated Lie algebras without Serre relations, weights, integrable modules, roots, the categories ${\mathcal O}$ and $\widetilde{{\mathcal O}}$, Serre relations, connections between representation theories of $\glie$ and $\tglie$, the Weyl group and some of its actions, the Harish-Chandra map, the category $\Owg$, filtrations of modules in ${\mathcal O}$. \\

The construction of first Yoneda extension groups, without proof, is recalled. The construction of higher ones is omitted since we do not use them in this work. We express how Yoneda Ext groups give a realisation of abstract Ext groups. We explain moreover how one can give vectorial space structures, and describe them, to the former from the latter. Finally, we give a first illustration of the use of Yoneda first Ext groups: see lemma \ref{lem_Ytglie}. For details about Yoneda Ext groups, a modern reference is \cite{McL}.


\subsection{Notations and conventions}
We denote by $\KK$ a (commutative) field. Except when dealing with Kac-Moody algebras, no assumption is made about the characteristic of $\KK$. \\

All the vector spaces, the (associative) algebras and the Lie algebras are considered over $\Bbbk$. For a vector space $V$, $V^{\ast}$ designates the vector space $\text{Hom}_{\KK}(V,\KK)$. \\

The modules (over an associative algebra or over a Lie algebra) will be left. For a Lie algebra $\alie$, its universal enveloping algebra is as usual denoted by $U(\alie)$ and the adjoint representation by $\text{ad}: \alie \to \text{End}_{\KK}(\alie)$. We recall the datum of an $\alie$-module is equivalent to the datum of a $U(\alie)$-module. \\

Ext groups, Tor groups and (co)homology groups of $\alie$-modules are handled as vector spaces and vanish by convention in negative degrees.

\subsection{Characters} \label{subs_ch}
We recall the goal of this subsection is to give some basic results about generalised eigenspaces related to characters: see lemma \ref{lem_trigonalizable}. Characters, eigenspaces and generalised eigenspaces in a module associated to a character are defined in \ref{para_ch}.


\subsubsection{} \label{para_ch}
Let $A$ be an associative algebra, $B$ a commutative subalgebra of $A$ and $M$ an $A$-module. Let $\alpha \in B^{\ast}$, denote:
$$ M_{\alpha} \ := \ \bigcap_{x \in B} M_{x,\alpha(x)} \, , \quad \ M^{\infty}_{\alpha} \ := \ \bigcap_{x \in B} M^{\infty}_{x,\alpha(x)} \, ; $$
$$ M_{x,\lambda} \ := \ \Big \{ m \in M \, , \ x.m = \lambda \, m \Big\} \, \quad (x \in B, \lambda \in \KK) \, , $$
$$ M^{\infty}_{x,\lambda} \ := \ \Big \{ m \in M \, , \ \big(x - \lambda \big)^k.m = 0 \ \text{ for some } k \in \NN \Big \} \, \quad (x \in B, \lambda \in \KK) \, . $$
Remark that $M_{\alpha} \subset M^{\infty}_{\alpha}$. \\

If $M^{\infty}_{\alpha} \neq 0$ (in particular if $M_{\alpha} \neq 0$), then $\alpha$ is automatically a character of $B$, i.e. $\alpha$ is a morphism of algebra from $B$ to $\KK$, since:
$$ xy - \lambda \beta \ = \ x(y - \beta) + \beta(x- \lambda) \, , \quad \ \forall \, x,y \in B, \ \forall \, \lambda, \beta \in \KK \, . $$ \\
Let $\alpha$ be a character of $B$. The vector subspaces $M_{\alpha}$ and $M^{\infty}_{\alpha}$ of $M$ are respectively called the $B$-eigenspace and the generalised $B$-eigenspace of $M$ associated to $\alpha$.
The dimensions of $M_{\alpha}$ and $M^{\infty}_{\alpha}$ are respectively called the multiplicity and the generalised multiplicity of $\alpha$ in $M$. \\

$M$ is said to be $B$-diagonalizable ($B$-trigonalizable) if $M$ is equal to the sum of its $B$-eigenspaces (generalised $B$-eigenspaces). \\

Note the $B$-eigenspaces and the generalised $B$-eigenspaces of $M$ are $B$-submodules of $M$. If $B$ is included in the center of $A$, then they are $A$-submodules of $M$.


\subsubsection{}
We give in lemma \ref{lem_trigonalizable} the results about characters and associated generalised eigenspaces, which will be used in this work. Lemma \ref{lem_diagonalizable} is the analog for eigenspaces. Note however that point 5 of lemma \ref{lem_trigonalizable} has no analog, it is in fact an advantage of generalised eigenspaces, we will benefit from.

\begin{lem} \label{lem_trigonalizable}
Let $\alpha$ be a character of $B$ and let $M,N$ be two $B$-trigonalizable $A$-modules.
\begin{enumerate}
\item[1)] Let $x \in B$. The action of $x$ on $M$ is locally finite.
\item[2)] The sum of the generalised $B$-eigenspaces of $M$ is direct.
\item[3)] Every $A$-submodule $M_1$ of $M$ is $B$-trigonalizable. \\
Moreover the generalised multiplicity of $\alpha$ in $M_1$ is less than or equal to the generalised  multiplicity of $\alpha$ in $M$.
\item[4)] Every $A$-quotient $M_2$ of $M$ is $B$-trigonalizable. \\
Moreover the generalised multiplicity of $\alpha$ in $M_2$ is less than or equal to the generalised multiplicity of $\alpha$ in $M$.
\item[5)] Every extension $E$ of $N$ by $M$ is $B$-trigonalizable. \\
Moreover the generalised multiplicity of $\alpha$ in $E$ is the sum of the generalised multiplicities of $\alpha$ in $M$ and $N$.
\end{enumerate}
\end{lem}

\proof
\begin{enumerate}
\item[1)] The action of $x$ on $M$ is locally finite since it is on each generalised $B$-eigenspace of $M$.
\item[2)] Let $x \in B$. The sum of the generalised eigenspaces of a linear operator acting on a finite-dimensional space is direct. Thanks to point 1, we thus have:
\begin{equation} \label{eq_mprime}
M \ = \ \bigoplus_{\lambda \in \KK} \, M^{\infty}_{x,\lambda} \, .
\end{equation}
Since we have \eqref{eq_mprime} for all $x \in B$, we can conclude:
$$ M \ = \ \bigoplus_{\alpha \in B^{\ast}} M^{\infty}_{\alpha} \, . $$
\item[3)] Let $x \in B$. The restriction to a stable vector subspace of a trigonalizable linear operator, acting on a finite-dimensional vector space, remains trigonalizable. Thanks to point 1, the action of $x$ on $M_1$ thus remains trigonalizable. This being true for all $x \in B$, $M_1$ is $B$-trigonalizable. \\
The statement about generalised multiplicities is straightforward.
\item[4)] Clear.
\item[5)] We have an exact sequence of $A$-modules:
$$ \xymatrix{ 0 \ar[r] & M \ar[r]^i & E \ar[r]^{p} & N \ar[r] & 0 \, . } $$
Let $x \in B$. Since the action of $x$ is locally finite on both $M$ and $N$ (thanks to point 1), so it is on the extension $E$. Let $v \in E$ and $V$ a finite-dimensional subspace of $E$ which contains $v$ and which is stabilized by $x$. Denote by $B'$ the subalgebra of $B$ generated by $x$. \\
Since $i(M) \cap V$ is a $(B')$-submodule of $i(M)$ and since $V / (i(M) \cap V)$ can be identified through $p$ with a $(B')$-submodule of $N$, points 3 and 4 (consider the inclusion of algebras $B' \subset A$) imply that $i(M) \cap V$ and $V / (i(M) \cap V)$ are $(B')$-trigonalizable. \\
 $V$ is thus an extension of two finite-dimensional vector spaces on which the induced actions of $x$ are trigonalizable. Then the action of $x$ on $V$ is trigonalizable. \\
It follows that the action of $x$ on $E$ is trigonalizable. This being true for all $x \in B$, we have proved that $E$ is $B$-trigonalizable. \\
The statement about generalised multiplicities is straightforward.
\end{enumerate}
\qed \\

One has a $B$-diagonalizable version of the first four points of lemma \ref{lem_trigonalizable}. It can be seen as a direct corollary of the latter.

\begin{lem} \label{lem_diagonalizable}
Let $\alpha$ be a character of $B$ and let $M,N$ be two $B$-diagonalizable $A$-modules.
\begin{enumerate}
\item[1)] Let $x \in B$. The action of $x$ on $M$ is locally finite.
\item[2)] The sum of the $B$-eigenspaces of $M$ is direct.
\item[3)] Every $A$-submodule $M_1$ of $M$ is $B$-diagonalizable. \\
Moreover the multiplicity of $\alpha$ in $M_1$ is less than or equal to the multiplicity of $\alpha$ in $M$.
\item[4)] Every $A$-quotient $M_2$ of $M$ is $B$-diagonalizable. \\
Moreover the multiplicity of $\alpha$ in $M_2$ is less than or equal to the multiplicity of $\alpha$ in $M$.
\end{enumerate}
\end{lem}



\subsection{Kac-Moody algebras} \label{subs_kac}
We recall here definitions related to Kac-Moody algebras and introduce notations and facts related to Kac-Moody algebras without Serre relations. \\
The topics tackled are generalised Cartan matrices, the definition of Kac-Moody algebras, some basic results about their structures, the associated Lie algebras without Serre relations, weights, integrable modules, roots, the categories ${\mathcal O}$ and $\widetilde{{\mathcal O}}$, Serre relations, connections between representation theories of $\glie$ and $\tglie$, the Weyl group and some of its actions, the Harish-Chandra map, the category $\Owg$, filtrations of modules in ${\mathcal O}$. \\
We recall the reader is referred to \cite{Kac} and \cite{KumBook} for details. \\

We assume the characteristic of $\KK$ is zero.

\subsubsection{}
Denote by $I$ a non empty finite set and denote by $l \in \NN^{\ast}$ its cardinality. A generalised Cartan matrix is a square matrix (of finite order) $A = (a_{ij})_{i,j \in I}$ with integral coefficients satisfying:
\begin{enumerate}
\item[a)] $a_{ii} = 2$ for all $i \in I$;
\item[b)] $a_{ij} \leq 0$ for all $i \neq j$ in $I$;
\item[c)] $a_{ij} = 0 \Leftrightarrow a_{ji} = 0$ for all $i,j \in I$.
\end{enumerate}
$A$ is said symmetrizable if there exists a $I$-tuplet of positive integers $(d_i)_{i \in I}$ such that:
$$ d_i \: \! a_{ij} \ = \ d_j \: \! a_{ji} \, , \quad \forall \, i,j \in I \, . $$


\subsubsection{}
Choose a triple $(\hlie,\pi, \pi^{\vee})$ where $\hlie$ is a vector space of dimension $(l + \text{corank} \, A)$ and where $\pi, \pi^{\vee}$ are families of linearly independent elements indexed by $I$, respectively contained in $\hlie^{\ast}$ and $\hlie$ and respectively called simple roots and simple coroots:
$$ \pi \ =: \ \{ \alpha_i \}_{i \in I} \, , \quad \quad \pi^{\vee} \ =: \ \{ \alpha^{\vee}_i \}_{i \in I} \, . $$
Assume moreover than:
$$ \alpha_j(\alpha_i^{\vee}) \ = \ a_{ij} \, . $$
Such a triple, called a realisation of $A$, exists and is unique up to isomorphism. \\

The Kac-Moody algebra $\glie(A)$, which will be abbreviated to $\glie$, is the Lie algebra generated by the vector space $\hlie$, the generators $e_i, f_i$ ($i \in I$), with the defining relations ($\delta_{ij}$ designates the Kronecker symbol associated to the elements $i,j$):
\begin{equation} \label{eq_km1}
[\hlie, \hlie] \ = \ 0 \, ;
\end{equation}
\begin{equation} \label{eq_km2}
[h, e_i] \ = \ \alpha_i(h) \: \! e_i \, , \quad [h, f_i] \ = \ - \alpha_i(h) \: \! f_i \quad \quad (i \in I) \, ;
\end{equation}
\begin{equation} \label{eq_km3}
[e_i, f_j] \ = \ \delta_{ij} \, \alpha_i^{\vee} \quad \quad (i,j \in I) \, ;
\end{equation}
\begin{equation} \label{eq_km4} \tag{positive Serre relations}
(\text{ad} \, e_i)^{1 - a_{ij}} (e_j) \ = \ 0 \quad \quad (i,j \in I, \, i \neq j) \, ;
\end{equation}
\begin{equation} \label{eq_km5} \tag{negative Serre relations}
(\text{ad} \, f_i)^{1 - a_{ij}} (f_j) \ = \ 0 \quad \quad (i,j \in I, \, i \neq j) \, .
\end{equation}
If $A$ is symmetrizable, $\glie$ is called a symmetrizable Kac-Moody algebra. \\

Denote by $\tglie(A)$ or $\tglie$ the Lie algebra generated by the vector space $\hlie$, the generators $e_i, f_i$ ($i \in I$), subject only to the relations \eqref{eq_km1}, \eqref{eq_km2} and \eqref{eq_km3}. \\
$\tglie$ is called a Kac-Moody algebra without Serre relations. \\
Denote by $[\cdot, \cdot]_{\glie}$ and $[\cdot, \cdot]_{\tglie}$ the respective Lie products of $\glie$ and $\tglie$.


\subsubsection{}
The canonical maps $\hlie \to \glie$ and $\hlie \to \tglie$ are injective. Thus we can see $\hlie$ as a Lie subalgebra of both $\glie$ and $\tglie$. By the PBW theorem, we also can see $U(\hlie)$ as a subalgebra of both $U(\glie)$ and $U(\tglie)$. \\

$(U(\hlie))$-eigenspaces and generalised $(U(\hlie))$-eigenspaces of a $\glie$-module or $\tglie$-module are respectively called the weight spaces and the generalised weight spaces. \\
Note that a character $\lambda: U(\hlie) \to \KK$ is uniquely determined by its linear restriction to $\hlie$. Thus we can see characters of $U(\hlie)$ as elements in $\hlie^{\ast}$. \\

Let $M$ be a $\glie$-module or a $\tglie$-module and let $\lambda \in \hlie^{\ast}$. \\
$M$ is said to be $\hlie$-diagonalizable ($\hlie$-trigonalizable) if $M$ is $(U(\hlie))$-diagonalizable ($(U(\hlie))$-trigonalizable). A $\hlie$-diagonalizable module will be also called a weight module. \\

If the multiplicity (generalised multiplicity) of $\lambda$ in $M$ is nonzero, then $\lambda$ is called a weight (generalised weight) of $M$. \\
The set of weights of $M$ is denoted by $\wt M$. The set of generalised weights of $M$ is denoted by $\wtf (M)$. Remark that $\wt M \subset \wtf (M)$.


\subsubsection{}
Denote by $\nlie^+$ and by $\nlie^-$ the Lie subalgebras of $\glie$ respectively generated by $\{e_i, \, i \in I \}$ and by $\{f_i, \, i \in I \}$. \\
Denote by $\tnlie^+$ and by $\tnlie^-$ the Lie subalgebras of $\tglie$ respectively generated by $\{e_i, \, i \in I \}$ and by $\{f_i, \, i \in I \}$. \\

There are triangular decompositions of $\glie$ and $\tglie$:
\begin{equation} \label{eq_triangl}
\glie \ = \ \nlie^- \oplus \hlie \oplus \nlie^+ \, , \quad \quad \tglie \ = \ \tnlie^- \oplus \hlie \oplus \tnlie^+ \, .
\end{equation}
$\nlie^+$ and $\nlie^-$ are respectively subject only to the \eqref{eq_km4} and to the \eqref{eq_km5}. $\tnlie^+$ and $\tnlie^-$ are free Lie algebras. \\

Denote:
$$ Q^{\pm} \ := \ \left \{ \sum_{i \in I} \, n_i \: \! \alpha_i \, , \ \pm \, n_i \in \NN \right \} \ \subset \ \hlie^{\ast} \, . $$
$Q^+$ and $Q^-$ are respectivey called the positive root lattice and the negative root lattice. $Q:= Q^- \cup Q^+$ is called the root lattice. \\

As a $\glie$-module ($\tglie$-module) under the adjoint action, $\glie$ ($\tglie$) is $\hlie$-diagonalizable. Moreover, for any $\alpha \in Q$, $\dim \glie_{\alpha} < \infty$ and $\dim \tglie_{\alpha} < \infty$. \\
There are root space decompositions:
\begin{equation} \label{eq_rootg}
\nlie^{\pm} \ = \ \bigoplus_{\alpha \in Q^{\pm}} \glie_{\alpha} \, , \quad \quad \hlie \ = \ \glie_0 \, ;
\end{equation}
\begin{equation} \label{eq_rootgt}
\tnlie^{\pm} \ = \ \bigoplus_{\alpha \in Q^{\pm}} \tglie_{\alpha} \, , \quad \quad \hlie \ = \ \tglie_0 \, .
\end{equation}
The nonzero weights of $\glie$ are called the roots of $\glie$. The set of roots is denoted by $\Delta$. Note that $\Delta$ is contained in $Q$. Thus $\Delta = \Delta^- \sqcup \Delta^+$, where $\Delta^{\pm}:= \Delta \cap Q^{\pm}$. The Cartan involution symmetry (see \ref{para_Cartaninv}) implies that $\Delta^- = - \Delta^+$.


\subsubsection{} \label{para_Cartaninv}
Denote by $\omega: \glie \toiso \glie$ and by $\tilde \omega: \tglie \toiso \tglie$ the automorphisms of the Lie algebras respectively $\glie$ and $\tglie$, which send $e_i$ to $f_i$, $f_i$ to $e_i$ ($i \in I$) and $h$ to $-h$ ($h \in \hlie$). These automorphisms are called the Cartan involutions. \\

Let $M$ be a $\glie$-module. \\
Denote by $M^{\omega}$ the $\glie$-module whose underlying vector space is still $M$ and where the action by $\glie$ has been twisted by $\omega$. \\
Denote by $M^{\vee}$ the left $\glie$-module whose underlying space is the $\hlie$-diagonalizable part $M^{\hlie}$ (i.e. the sum of the weight spaces of $M^{\ast}$) of the $\glie$-module $M^{\ast}$ and where the action by $\glie$ has been twisted by $\omega$.


\subsubsection{} \label{para_Ocat}
Let $\lambda, \mu \in \hlie^{\ast}$. Define a partial order $\leq$ in $\hlie^{\ast}$ by $\mu \leq \lambda$ if $\lambda - \mu \in Q^+$. \\
Denote by $D(\lambda)$ the set $\{ \mu \in \hlie^{\ast} , \, \mu \leq \lambda \}$. \\
Denote by $D^<(\lambda)$ the set $\{ \mu \in \hlie^{\ast} , \, \mu < \lambda \}$. \\
Denote by $D^{\geq}(\lambda)$ the set $\{ \mu \in \hlie^{\ast} , \, \mu \geq \lambda \}$. \\
Denote by $D^>(\lambda)$ the set $\{ \mu \in \hlie^{\ast} , \, \mu > \lambda \}$. \\

A highest weight $\glie$-module ($\tglie$-module) $M$ is a $\glie$-module ($\tglie$-module) generated by a weight vector, which is $(\nlie^+)$-invariant ($(\tnlie^+)$-invariant). \\
Remark that $M$ is a weight module with finite-dimensional weight spaces and that $\wt M \subset D(\lambda)$, where $\lambda$ is the weight of the highest weight vector. \\

Among all highest weight $\glie$-modules ($\tglie$-modules) $M$ of highest weight $\lambda \in \hlie^{\ast}$, there is an universal one, namely the Verma module denoted by $M(\lambda)$ ($\tilde M(\lambda)$): $M$ is a quotient of $M(\lambda)$ ($\tilde M(\lambda)$). \\
Moreover any highest weight module has a unique simple quotient, denoted by $L(\lambda)$ ($\tilde L(\lambda)$). \\

Denote respectively by ${\mathcal O}$ and $\widetilde{{\mathcal O}}$ the categories of $\glie$-modules and $\tglie$-modules $M$ satisfying the following:
\begin{enumerate}
\item[\textbullet] $M$ is a weight module with finite-dimensional weight spaces;
\item[\textbullet] there exist finitely many $\lambda_1, \dots, \lambda_k \in \hlie^{\ast}$ such that $\wt M \subset \bigcup_{s=1}^k D(\lambda_s)$.
\end{enumerate}
The morphisms in ${\mathcal O}$ (in $\widetilde{{\mathcal O}}$) are all $\glie$-module ($\tglie$-module) morphisms. \\

Let $M$ be in ${\mathcal O}$ and $\lambda \in \hlie^{\ast}$. \\
$L(\lambda)$ is said to be a component of $M$ if it appears as a subquotient of $M$. \\

A $\glie$-module ($\tglie$-module) is said integrable if the actions of $e_i$ and $f_i$ are locally nilpotent for all $i \in I$. Integrability implies Serre relations: the action of $\tglie$ on a integrable $\tglie$-module factorizes through $\glie$: see \ref{para_gtildeg} \\

Denote by ${\mathcal O^{\mathrm{int}}}$ the full subcategory of ${\mathcal O}$ whose modules are integrable. The category ${\mathcal O^{\mathrm{int}}}$ is semisimple and its simple objects are the modules $L(\lambda)$ with $\lambda$ dominant (i.e. $\langle \lambda, \alpha_i^{\vee} \rangle \in \NN$ for all $i \in I$). If $\glie$ is finite-dimensional, ${\mathcal O^{\mathrm{int}}}$ is actually the category of finite-dimensional $\glie$-modules. \\

A weight $\lambda \in \hlie^{\ast}$ is said integral if $\langle \lambda, \alpha_i^{\vee} \rangle \in \ZZ$ for all $i \in I$. The set of integral weights is denoted by $\hlie^{\ast}_{\ZZ}$.


\subsubsection{} \label{para_slie}
Denote by $\prg: \tglie \to \glie$ the canonical Lie algebra projection. \\
Denote by $\tslie^+$ and $\tslie^-$ the Lie ideals of respectively $\tnlie^+$ and $\tnlie^-$, respectively generated by the positive Serre relations $u_{ij}^+$ ($i \neq j$ in $I$) and by the negative Serre relations $u_{ij}^-$ ($i \neq j$ in $I$):
$$ u_{ij}^+ \ := \ (\text{ad} \, e_i)^{1 - a_{ij}} (e_j) \, , \quad \quad u_{ij}^- \ := \ (\text{ad} \, f_i)^{1 - a_{ij}} (f_j) \, . $$
Actually $\tslie^{\pm}$ is also a Lie ideal of $\tglie$. It is a consequence of the following:
$$ \Big[ e_k \, , \, u_{ij}^- \Big]_{\tglie} \ = \ \Big[ f_k \, , \, u_{ij}^+ \Big]_{\tglie} \ = \ 0 \, , \quad \ \forall \ i,j,k \in I, \ i \neq j \, . $$
Denote by $\tslie:= \tslie^- \oplus \tslie^+$ the Serre relations ideal of $\tglie$. Remark the Lie algebra $\glie$ is isomorphic to the Lie quotient $\tglie / \tslie$.


\subsubsection{} \label{para_gtildeg}
We give here some known connections between representation theories of $\glie$ and $\tglie$. No particular references are given but proofs are either straightforward, explained or can be easily completed from basics of category ${\mathcal O}$ and of $\mathfrak{sl}_2$ representation theory.

\begin{enumerate}
\item[\textbullet] First, remark that any $\glie$-module is a $\tglie$-module by restriction.
\item[\textbullet] Any integrable $\tglie$-module is actually the restriction of a $\glie$-module. \\
Let us explain it. We have to prove the Serre relations are satisfied in an integrable $\tglie$-module $M$. Fix $i, j \in I$ with $i \neq j$ and denote by $x^M$ the image in $\text{End}_{\KK}(M)$ of an element $x \in \tglie$. In another hand, $\text{End}_{\KK}(M)$ is a $\tglie$-module and one has:
\begin{equation} \label{eq_serreint1}
e_i . (f_j^M) \ = \ \Big[ e^M_i,f^M_j \Big] \ = \ \Big( [e_i, f_j] \Big)^M \ = \ 0 \, ,
\end{equation}
\begin{equation} \label{eq_serreint2}
\alpha^{\vee}_i. (f_j^M) \ = \ \Big[ (\alpha^{\vee}_i)^M,f^M_j \Big] \ = \ \Big( [\alpha^{\vee}_i, f_j] \Big)^M \ = \ -a_{ij} \, f_j^M \, .
\end{equation}
The actions of $f_i$, $e_i$ and $\alpha^{\vee}_i$ endow $M$ and $\text{End}_{\KK}(M)$ with $(\mathfrak{sl}_2)$-module structures. Since $M$ is integrable, it is locally finite as a $(\mathfrak{sl}_2)$-module and then so is $\text{End}_{\KK}(M)$. Considering the finite-dimensional highest weight $(\mathfrak{sl}_2)$-submodule of $\text{End}_{\KK}(M)$ generated by $f_j^M$ and thanks to \eqref{eq_serreint1} and \eqref{eq_serreint2}, one has:
$$ \Big( \text{ad}_{f_i}^{1-a_{ij}}(f_j) \Big)^M \ = \ (f_i^{\, a_{ij}+1}) . (f_j^M) \ = \ 0 \, . $$
In other words, the negative Serre relation $u_{ij}^-$ is satisfied in $M$. The proof for positive Serre relations is similar (or one can use the Cartan involution $\tilde \omega$, see \ref{para_Cartaninv}). \\
Note that, as a direct consequence, a finite-dimensional $\tglie$-module is the restriction of a $\glie$-module.
\item[\textbullet] A simple $\tglie$-module in $\widetilde{{\mathcal O}}$ is actually the restriction of a $\glie$-module in ${\mathcal O}$. This follows from the fact that a simple module in $\widetilde{{\mathcal O}}$ is of highest weight, thus a quotient of a Verma module, and from the fact that Verma modules in both ${\mathcal O}$ and $\widetilde{{\mathcal O}}$ have a unique simple quotient (thus the same).
\end{enumerate}


\subsubsection{}
For any $i \in I$, one defines the reflection $s_i \in \text{Aut}_{\KK} (\hlie^{\ast})$ by:
$$ s_i (\chi) \ := \ \chi \, - \, \langle \chi, \alpha_i^{\vee} \rangle \, \alpha_i \, , \quad \quad (\chi \in \hlie^{\ast}) \, . $$
The Weyl group associated to $\glie$ is the subgroup $W \subset \text{Aut}_{\KK} (\hlie^{\ast})$ generated by $s_i$ ($i \in I$). \\

Let $\rho \in \hlie^{\ast}$ such that $\langle \rho, \alpha_i^{\vee} \rangle = 1$ for all $i \in I$. The shifted action of $W$ on $\hlie^{\ast}$ is defined by:
$$ w \ast \lambda \ := \ w(\lambda + \rho) \, - \, \rho \, \quad \quad (w \in W, \ \lambda \in \hlie^{\ast}) \, . $$
The definition does not depend on the choice of $\rho$. The equivalence relation induced by the shifted action is denoted by $\sim^W$. \\

A root $\alpha \in \Delta$ is called real if $\alpha = w(\alpha_i)$ for some $w \in W$ and $i \in I$. It is called imaginary otherwise. The set of real roots is denoted by $\Delta_{\text{re}}$, the set of imaginary roots by $\Delta_{\text{im}}$. One defines: $\Delta^{\pm}_{\text{re}}:= \Delta_{\text{re}} \cap Q^{\pm}$ and $\Delta^{\pm}_{\text{im}}:= \Delta_{\text{im}} \cap Q^{\pm}$.


\subsubsection{}
We recall here definition of Harish-Chandra map, which allows one to express the following statement: the center of $U(\glie)$ separates the Weyl orbits. This fact will be used in the proof of propositon \ref{prop_extpos}. \\

Denote by $Z_U(\glie)$ the center of $U(\glie)$. A character $Z_U(\glie) \to \KK$ is called a central character of $\glie$. \\

The triangular decomposition \eqref{eq_triangl} gives rise to the decomposition:
$$ U(\glie) \ = \ \Big( (\nlie^-) \, U(\glie) \, + \, U(\glie) \, (\nlie^+) \Big) \, \oplus \, U(\hlie) \, . $$
This induces a projection $\mathcal H: U(\glie) \to U(\hlie)$ called the Harish-Chandra map. \\

Denote by $\mathcal H_Z: Z_U(\glie) \to U(\hlie)$ the restriction of $\mathcal H$ to the center of $U(\glie)$. $\mathcal H_Z$ is a morphism of (unital) algebra. \\

If $\glie$ is finite-dimensional, then $\mathcal H_Z$ separates the Weyl orbits (recall that we identify the characters of $U(\hlie)$ with the elements of $\hlie^{\ast}$):
$$ \lambda \sim^W \mu \ \Longleftrightarrow \ \lambda \circ \mathcal H_Z \ = \ \mu \circ \mathcal H_Z \, , \quad \quad (\lambda, \mu \in \hlie^{\ast}) \, . $$
In the infinite-dimensional case, only the direct implication remains valid. \\

Let $V$ be a highest weight $\glie$-module of highest weight $\lambda$. \\
The action of $Z_U(\glie)$ on $V$ is scalar and given by $x.v = (\lambda \circ \mathcal H) (x) \, v$ ($x \in Z_U(\glie)$, $v \in V$).


\subsubsection{}
We recall here useful lemmas. For a proof of them, see for example \cite[lemmas 2.1.9 \& 2.1.10]{KumBook}.

\begin{lem} \label{lem_finiteseq}
Let $M$ be in ${\mathcal O}$ and let $\lambda \in \hlie^{\ast}$. \\
There exists a filtration $0 = M_0 \subset M_1 \subset M_2 \subset \cdots \subset M_p = M$ by $\glie$-submodules ($p \in \NN$) such that each $V_k:= M_{k+1} / M_k$ ($0 \leq k \leq p-1$) satisfies at least one of the following:
\begin{enumerate}
\item[i)] $V_k$ is simple with highest weight $\lambda_k \geq \lambda$;
\item[ii)] $(V_k)_{\mu} = 0$ for all $\mu \in D^{\geq}(\lambda)$.
\end{enumerate}
\end{lem}

\begin{lem} \label{lem_hwseq}
Let $M$ be in ${\mathcal O}$. \\
There exists a (possibly infinite) increasing filtration $0 = M_0 \subset M_1 \subset M_2 \subset \cdots$ by $\glie$-submodules of $M$ such that:
\begin{enumerate}
\item[i)] $\bigcup_{k \in \NN} M_k = M$;
\item[ii)] $M_{k+1} / M_k$ is a highest weight module, for all $k \in \NN$.
\end{enumerate}
\end{lem}

%Let $M$ be a $\hlie$-diagonaizable $\glie$-module, whose weight spaces are finite-dimensional. \\
%Denote by $e_{\lambda} \in \NN^{\hlie^{\ast}}$ ($\lambda \in \hlie^{\ast}$) the map from $\hlie^{\ast}$ to $\NN$ defined by $e_{\lambda}(\lambda) = 1$ and $e_{\lambda}(\mu) = 0$ if $\mu \neq \lambda$. \\
%We define the formal character of $M$ by:
%$$ \text{ch} \, M \ := \ \sum_{\lambda \in \hlie^{\ast}} (\dim M_{\lambda}) \, e_{\lambda} \ \in \ \NN^{\hlie^{\ast}} \, . $$

%A family of elements $(a_k \in \NN^{\hlie^{\ast}}, \, k \in K)$ ($K$ is a set) is called locally finite if for any $\lambda \in \hlie^{\ast}$, the set $K_{\lambda}:= \{ k \in K, \, a_k(\lambda) \neq 0 \}$ is finite. \\
%In this case, the sum $\sum_{k \in K} a_k$ clearly makes sense in $\NN^{\hlie^{\ast}}$.

%\begin{lem} \label{lem_chcomp}
%Let $M \in {\mathcal O}$. \\
%There exist a unique family of integers $[M: L(\lambda)] \in \NN$ (called the multiplicity of $L(\lambda)$ in $M$), indexed by $\lambda \in \hlie^{\ast}$, such that:
%\begin{enumerate}
%\item[i)] for all $\lambda \in \hlie^{\ast}$, $[M: L(\lambda)] \neq 0$ if and only if $L(\lambda)$ is a component of $M$;
%\item[ii)] $\Big( [M: L(\lambda)] \, \text{ch} \, L(\lambda) \Big), \, \lambda \in \hlie^{\ast})$ is locally finite;
%\item[iii)] $\text{ch} \, M = \sum_{\lambda \in \hlie^{\ast}} [M: L(\lambda)] \, \text{ch} \, L(\lambda)$.
%\end{enumerate}
%\end{lem}


\subsubsection{} \label{para_wg}
In \cite{DGK}, Deodhar, Gabber and Kac defined a subcategory ${\mathcal O}^{\text g}$ of ${\mathcal O}$ in order to generalise, in the (symmetrizable) Kac-Moody infinite-dimensional case, results known for the category ${\mathcal O}$ of  a finite-dimensional semisimple Lie algebra. Note that g stands for good. In \cite{KumO}, Kumar defined an extension $\Owg$ of ${\mathcal O}^{\text g}$, where main results of \cite{DGK} remain valid. Here wg stands for weakly good. \\

We recall here the related definitions. We assume that $\glie$ is symmetrizable. \\

Let $\alpha \in \Delta^+_{\text{im}}$ and define $C_{\alpha}:= \{ \lambda \in \hlie^{\ast} , \, \langle \lambda + \rho, \alpha \rangle = \langle \alpha, \alpha \rangle / 2 \}$, $C:= \bigcup_{\alpha \in \Delta_{\text{im}}^+} C_{\alpha}$. Define $K^{\text{wg}}:= \hlie^{\ast} \backslash C$. All dominant weights belong to $K^{\text{wg}}$. Moreover if $\lambda \in K^{\text{wg}}$ and if $\mu \sim^W \lambda$, then $\mu \in K^{\text{wg}}$. \\

$\Owg$ is the full subcategory of ${\mathcal O}$ consisting of all those modules $M$ in ${\mathcal O}$ such that all the components $L(\lambda)$ ($\lambda \in \hlie^{\ast}$) of $M$ satisfy $\lambda \in K^{\text{wg}}$. \\

Define a relation $\to$ in $\hlie^{\ast}$ by $\lambda \to \mu$ if $L(\lambda)$ is a component of $M(\mu)$. Let $\sim$ be the equivalence relation in $\hlie^{\ast}$ generated by $\to$. \\
Let $\to^0$ be the restriction of $\to$ to $K^{\text{wg}}$ and let $\sim^0$ be the equivalence relation in $K^{\text{wg}}$ generated by $\to^0$. \\
Of course $\lambda \sim^0 \mu \Rightarrow \lambda \sim \mu$ ($\lambda, \mu \in K^{\text{wg}}$). The converse does not hold in general. \\

If $\lambda$ and $\mu$ are two dominant weights, then $\lambda \sim^0 \mu$ is equivalent to $\lambda = \mu$. \\

Let $\Lambda \subset \hlie^{\ast}$ and $\Lambda^0 \subset K^{\text{wg}}$ be equivalence classes respectively under $\sim$ and $\sim^0$. The equivalence class of $0$ will be denoted by $0$ both in $\hlie^{\ast}$ and $K^{\text{wg}}$. \\
A module $M$ be in ${\mathcal O}$ (in $\Owg$) is said to be of type $\Lambda$ (of type $\Lambda^0$) if for all components $L(\lambda)$ of $M$, one has $\lambda \in \Lambda$ ($\lambda \in \Lambda^0$). \\
The categories ${\mathcal O}_{\Lambda}$ and $\Owg_{\Lambda^0}$ are respectively the full subcategories of ${\mathcal O}$ and $\Owg$, whose modules are respectively of type $\Lambda$ and $\Lambda^0$. ${\mathcal O}_{\Lambda}$ and $\Owg_{\Lambda^0}$ are called blocks of respectively ${\mathcal O}$ and $\Owg$. ${\mathcal O}_0$ and $\Owg_0$ are called the principal blocks. \\

A highest weight module of highest weight $\lambda$ is in ${\mathcal O}_{\Lambda}$ (in $\Owg_{\Lambda^0}$) if and only if $\lambda \in \Lambda$ ($\lambda \in \Lambda^0$). \\

One has the following implication:
$$ \lambda \sim^0 \mu \ \Rightarrow \ \lambda \sim^W \mu \ \quad (\lambda, \mu \in K^{\text{wg}}) \, . $$
In general the converse is false, but one has an equivalence if $\lambda$ (or $\mu$) is integral. \\

Note that in the the finite-dimensional case, one has:
$$ K^{\text{wg}} \ = \ \hlie^{\ast} \, , \quad \ \Owg \ = \ {\mathcal O} \, , \quad \ \sim \ = \ \sim^0 \, . $$



\subsection{Yoneda extension groups} \label{subs_yoneda}
In \cite{Yon}, Yoneda gave a realisation of Ext groups in terms of $n$-extensions ($n \in \NN$). A modern reference is for example \cite[chapter III]{McL}. \\

First Yoneda extension groups will be used in this work (see propositon \ref{prop_gleqdimext}) to handle in a concrete way (i.e. in terms of module extensions) the group structures of first abstract Ext groups and eventually prove the equality between second cohomology groups of $\glie$ and $\tglie$ (see theorem \ref{thm_coho2}). \\

The construction of first Yoneda extension groups, without proof, is recalled. The construction of higher ones is omitted since we do not use them in this work. We express how Yoneda Ext groups give a realisation of abstract Ext groups. We explain moreover how one can give vectorial space structures to the former from the latter. Note the author does not know any precise reference for this last point, all the (not complicated) details are thus given. Finally, we give a first illustration of the use of Yoneda first Ext groups: see lemma \ref{lem_Ytglie}. \\

Let $\alie$ be a Lie algebra. The Yoneda extension groups of modules over $\alie$ are denoted by $\text{YExt}_{\alie}^{\bullet}$. No assumption is made on the characteristic of $\KK$. \\

Let $M,M',N,N'$ be $\alie$-modules. Let $E$ and $E'$ be extensions of respectively $M$ by $N$ and $M'$ by $N'$. Denote respectively by $i$ and $i'$ the associated injective morphisms $N \to E$ and $N' \to E'$. Denote respectively by $p$ and $p'$ the associated surjective morphisms $E \to M$ and $E' \to M'$. \\
The datum of a morphism of $\alie$-module $\beta: E' \to E$ is equivalent to the datum of a triple $(\alpha, \beta, \gamma)$ of morphisms of $\alie$-module such that the following diagram commutes:
$$ \xymatrix{
0 \ar[r] & N' \ar[r] \ar[d]^{\alpha} & E' \ar[d]^{\beta} \ar[r] & M' \ar[r] \ar[d]^{\gamma} & 0 \ \, \\
0 \ar[r] & N \ar[r] & E \ar[r] & M \ar[r] & 0 \, .
} $$

The set of isomorphism classes of extensions $E$ (of $M$ by $N$) is denoted by $\text{YExt}_{\alie}^1(M,N)$. The product giving the abelian group structure to $\text{YExt}_{\alie}^1(M,N)$ is named the Baer sum. Let us recall the definition. \\

Let us fix $\gamma: M' \to M$ a morphism of $\alie$-module. \\
For each extension $E$ of $M$ by $N$ there exist an extension $E'$ of $M'$ by $N$ and a morphism of extension $(\text{id}_N, \beta, \gamma): E' \to E$. Moreover the pair $(E',\beta)$ is unique up to isomorphism. Any choice of such association $E \mapsto E'$ gives rise to the same application between Yoneda first extension groups, which we denote by:
\begin{equation} \label{eq_gamma}
\gamma^{\ast} \,: \ \text{YExt}_{\alie}^1 (M,N) \ \to \ \text{YExt}_{\alie}^1 (M',N) \, .
\end{equation}
Remark the notations for an extension and its isomorphism class are the same. Note that $\gamma^{\ast}$ is a group morphism when one consider the group structures on first Yoneda extension groups. \\

Let us fix $\alpha: N' \to N$ a morphism of $\alie$-module. \\
For each extension $E'$ of $M'$ by $N'$, there exist an extension $E$ of $M'$ by $N$ and a morphism of extension $(\alpha, \beta, \text{id}_{M'}): E' \to E$. Moreover the pair $(E,\beta)$ is unique up to isomorphism. Any choice of such association $E' \mapsto E$ gives rise to the same application between Yoneda extension groups, which we denote by:
$$ \alpha_{\ast} \,: \ \text{YExt}_{\alie}^1 (M',N') \ \to \ \text{YExt}_{\alie}^1 (M',N) \, . $$

Let $E_1$ and $E_2$ be two extensions of $M$ by $N$. Remark that $E_1 \oplus E_2$ is naturally an extension of $M \oplus M$ by $N \oplus N$. The Baer sum $E_1 + E_2$ is an extension of $M$ by $N$ given by:
\begin{eqnarray*}
E_1 + E_2 &:= & \Big( (\Delta_M)^{\ast} \circ (\nabla_{\! N})_{\ast} \Big) (E_1 \oplus E_2) \\
& = & \Big( (\nabla_{\! N})_{\ast} \circ (\Delta_M)^{\ast} \Big) (E_1 \oplus E_2) \, ,
\end{eqnarray*}
where $\nabla_{\! N}: N \oplus N \to N$ designates the addition application ($\nabla_{\! N}(x \oplus y) = x + y$) and $\Delta_M: M \to M \oplus M$ designates the diagonal application ($\Delta_M(x) = x \oplus x$). \\

As we have already mentioned, Yoneda extension groups are a realisation of abstract extension groups. More precisely, for all $\alie$-modules $M,N$ and for all $n \in \NN$, there exist group isomorphisms:
$$ \xi^n(M,N) \,: \ \text{YExt}_{\alie}^n(M,N) \ \toiso \ \text{Ext}_{\alie}^n (M,N) \, , $$
natural in $M$ (and in $N$ but we will not use this fact), i.e. for all group morphisms $\gamma: M' \to M$ and for all $n \in \NN$, the following diagram commutes:
\begin{equation} \label{eq_commgamma} \xymatrix{
\text{YExt}_{\alie}^n(M,N) \ar[rr]^{\xi^n(M,N)} \ar[d]_{\gamma^{\ast}} && \text{Ext}_{\alie}^n(M,N) \ar[d]_{\gamma^{\ast}} \\
\text{YExt}_{\alie}^n(M',N) \ar[rr]^{\xi^n(M',N)} && \text{Ext}_{\alie}^n(M',N)
} \end{equation}
At this matter, see \cite[theorem III.6.4]{McL}: the notation $\text{Ext}$ is used there to designate Yoneda extension groups. \\

Thanks to the isomorphisms $\xi^n$, one can carry vectorial space structures on Yoneda extension groups from abstract Ext groups, in a such way that $\xi^n$ becomes a linear isomorphism for all $n \in \NN$. Remark then that for $\gamma: M' \to M$, the application $\gamma^{\ast}$ evoked in \eqref{eq_gamma} becomes also linear, thanks to the commutative diagram \eqref{eq_commgamma}. \\

Fix $n \in \NN$. Given $\lambda \in \KK$, the multiplication by $\lambda$ in $\text{Ext}^n_{\alie}(M,N)$ is $m_{\lambda}^{\ast}$, where $m_{\lambda}$ is the multiplication by $\lambda$ in $M$. Thus, thanks again to the commutativity of \eqref{eq_commgamma}, the multiplication by $\lambda$ in $\text{YExt}^n_{\alie}(M,N)$ is:
$$ m_{\lambda}^{\ast} \,: \ \text{YExt}^n_{\alie}(M,N) \ \to \ \text{YExt}^n_{\alie}(M,N) \, . $$
From now, we consider Yoneda extension groups endowed with the previous vectorial space structures. \\

Let $\glie$ be a Kac-Moody algebra (assume the characteristic is zero). \\
In \ref{para_gtildeg}, we explained that an integrable $\tglie$-module is actually the restriction of a $\glie$-module. Thus, since an extension of two integrable modules is also integrable, we see the extensions study of integrable modules is the same in the two categories of $\glie$-modules and $\tglie$-modules. Yoneda first Ext groups allow us to make this equivalence more precise in the following lemma.

\begin{lem} \label{lem_Ytglie}
Let $M,N$ be two integrable $\glie$-modules. \\
There exists a natural linear isomorphism:
$$ \text{YExt}_{\glie}^1(M,N) \ \toiso \ \text{YExt}_{\tglie}^1(M,N) \, . $$
\end{lem}

\proof
Let $E$ be a $\tglie$-module, extension of $M$ by $N$. Since $M$ and $N$ are integrable, $E$ is also integrable. Thus the action of $\tglie$ on $E$ factorizes through $\glie$ (see \ref{para_gtildeg}). This induces a natural linear morphism:
$$ \text{YExt}_{\tglie}^1(M,N) \ \to \ \text{YExt}_{\glie}^1(M,N) \, . $$
In another hand, each $\glie$-module, extension of $M$ by $N$ can be seen by restriction as a $\tglie$-module, extension of $M$ by $N$. This induces a natural linear morphism:
$$ \text{YExt}_{\glie}^1(M,N) \ \toiso \ \text{YExt}_{\tglie}^1(M,N) \, . $$
It is clear that the two applications are inverses of each other.
\qed





\section{Relations between Cohomologies} \label{sect_ablie}
Let $\alie$ be a Lie algebra (no assumption is made on the characteristic of $\KK$, except when dealing with Kac-Moody algebras). Let $\ilie$ and $\jlie$ be two ideals of $\alie$ such that $[\ilie, \jlie] = 0$. We denote by $\blie$ the quotient Lie algebra $\alie / (\ilie \oplus \jlie)$. \\

In \ref{subs_ablie}, we relate to each other the cohomologies of the Lie algebras $\alie$ and $\blie$, with coefficients in a $\blie$-module $M$. Assuming that cohomological dimensions of ideals $\ilie$ and $\jlie$ are strictly less than 2, we use two times Hochschild-Serre spectral sequences by considering successively the two quotients $\alie':= \alie / \ilie$ and $\blie \simeq \alie' / \jlie$. Thanks to the hypothesis on cohomological dimensions of $\ilie$ and $\jlie$, most of the terms in the second sheets of the two spectral sequences vanish. In another hand, since assuming the coefficients space $M$ is a $\blie$-module, the non zero terms in the spectral sequences involve trivial $\ilie$-modules and trivial $\jlie$-modules, which lead to easy computations of intermediate cohomologies. As a consequence, we are able to compare, in a quite simple and concrete way, the dimensions of the cohomologies of $\alie$ and $\blie$ with coefficients in $M$. See proposition \ref{prop_ablie}. \\

The configuration (when assuming that cohomological dimensions of ideals $\ilie$ and $\jlie$ are strictly less than 2) of the Lie algebras couple $(\blie,\alie)$ will appear in \ref{subs_htilde} as a natural generalisation of the case we are interested in: $\blie$ is a Kac-Moody algebra, $\alie$ is the associated Lie algebra without Serre relations, $\ilie$ and $\jlie$ are the ideals of respectively negative and positive Serre relations. Proposition \ref{prop_ablie} will then give rise to theorem \ref{thm_htilde}.


\subsection{General case} \label{subs_ablie}
The ideals $\ilie$ and $\jlie$ of $\alie$ are left $\alie$-modules under the adjoint action of $\alie$. \\
$[\ilie, \ilie]$ and $[\jlie, \jlie]$ are respectively $\alie$-submodules of $\ilie$ and $\jlie$. The action of $\alie$ on the quotients $\ilie / [\ilie, \ilie]$ and $\jlie / [\jlie, \jlie]$ factorizes through $\blie$ since $[\ilie, \jlie] = 0$. \\
Denote then respectively by $I$ and by $J$ the $\blie$-modules $\ilie / [\ilie, \ilie]$ and $\jlie / [\jlie, \jlie]$. \\
Denote by $T$ the $\blie$-module $I \otimes_{\KK} J$.

\begin{prop} \label{prop_ablie}
Suppose that cohomological dimensions of $\ilie$ and $\jlie$ are strictly less than $2$. \\
Let $M$ be a $\blie$-module and let $n \in \NN$. Denote:
\begin{eqnarray*}
d_n &:= & \ \quad \dim \Big[ \text{Ext}_{\blie}^{\, n-1} (I, M) \Big] \ + \ \dim \Big[ \text{Ext}_{\blie}^{\, n-1} (J, M) \Big] \\
&& + \ \dim \Big[ \text{Ext}_{\blie}^{\, n-2} (T, M) \Big] \, ;
\end{eqnarray*}
\begin{eqnarray*}
d'_n &:= & \ \quad \dim \Big[ \text{Ext}_{\blie}^{\, n-2} (I, M) \Big] \ + \ \dim \Big[ \text{Ext}_{\blie}^{\, n-2} (J, M) \Big] \\
&& + \ \, 2 \: \! \dim \Big[ \text{Ext}_{\blie}^{\, n-3} (T, M) \Big] \, .
\end{eqnarray*}
The following inequality holds:
$$ d_n \ - \ d'_n \ \leq \ \dim \! \Big[ \text H^{\, n} (\alie,M) \Big] \ - \ \dim \! \Big[ \text H^{ \, n} (\blie,M) \Big] \ \leq \ d_n \, . $$
\end{prop}

\proof
Denote by $\alie'$ the Lie quotient $\alie / \ilie$. By abuse of notation, $\jlie$ will also designate the ideal $(\ilie \oplus \jlie) / \ilie$ of $\alie'$. Note that $\blie$ is naturally identified with the Lie quotient $\alie' / \jlie$. By restriction, one then can see $I$ as an $(\alie')$-module. \\

The proof will use in two steps the Hochschild-Serre spectral sequence (see \cite{HS}), by considering the following two successive canonical short exact sequences:
$$ 0 \ \longrightarrow \  \ilie \ \longrightarrow \  \alie \ \longrightarrow \  \alie ' \ \longrightarrow \  0 \, , $$
$$ 0 \ \longrightarrow \  \jlie \ \longrightarrow \  \alie ' \ \longrightarrow \  \blie \ \longrightarrow \  0 \, . $$
More precisely, for $N_1$ an $\alie$-module and $N_2$ an $(\alie ')$-module, one has two convergent spectral sequences:
\begin{equation} \label{eq_spectralseq1}
\text E^2_{p,q} \ = \ \text H^p \Big( \alie ' \, , \, \text H^q(\ilie, N_1) \Big) \ \Rightarrow \ \text H^{p+q}(\alie,N_1) \, ,
\end{equation}
\begin{equation} \label{eq_spectralseq2}
\text F^2_{p,q} \ = \ \text H^p \Big( \blie \, , \, \text H^q(\jlie, N_2) \Big) \ \Rightarrow \ \text H^{p+q}(\alie ',N_2) \, ,
\end{equation} \\

Let $N_1$ be an $\alie$-module and suppose the action of $\ilie$ on $N_1$ is trivial. Thus there exist isomorphisms of $(\alie')$-module:
\begin{equation} \label{eq_NH0}
\text H^0(\ilie, N_1) \ \simeq \ N_1 \, ;
\end{equation}
\begin{equation} \label{eq_NH1}
\text H^1(\ilie, N_1) \ \simeq \ \text{Hom}_{\KK}(I, N_1) \, .
\end{equation}
Note that in both right hand sides, $N_1$ is naturally seen as an $(\alie')$-module (recall the action of $\ilie$ on $N_1$ is trivial). $I$ is also seen as an $(\alie')$-module (see above). \\

Let $N_2$ be a $(\alie')$-module and suppose the action of $\jlie$ on $N_2$ is trivial. Thus there exist isomorphisms of $\blie$-module:
\begin{equation} \label{eq_NH0p}
\text H^0(\jlie, N_2) \ \simeq \ N_2 \, ;
\end{equation}
\begin{equation} \label{eq_NH1p}
\text H^1(\jlie, N_2) \ \simeq \ \text{Hom}_{\KK}(J, N_2) \, .
\end{equation} \\
Note that in both right hand sides, $N_2$ is naturally seen as a $\blie$-module (recall the action of $\jlie$ on $N_2$ is trivial). \\

By hypothesis, cohomological dimensions of $\ilie$ and $\jlie$ are strictly less than $2$. Since the actions of $\ilie$ and $\jlie$ on respectively $N_1$ and $N_2$ are trivial, one has:
\begin{equation} \label{eq_NH2}
\text H^q(\ilie, N_1) \ = \ 0 \, , \quad \ \text H^q(\jlie, N_2) \ = \ 0 \, , \quad \quad \forall \ q \geq 2 \, .
\end{equation} \\

By restriction the $\blie$-module $M$ can be seen as an $\alie$-module, where the action of $\ilie$ is then trivial. \\
Thanks to \eqref{eq_NH0} and \eqref{eq_NH2}, the second sheet of the spectral sequence \eqref{eq_spectralseq1} for $N_1 = M$, centered at degree $n-1$, looks like:
\begin{equation} \label{eq_2sheetspectralseq1} \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text H^{n-2} \Big( \alie' \, , \, \text H^1(\ilie, M) \Big) & \text E^{n-1,1}_2 \, = \, \text H^{n-1} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) & \text H^n \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \\
\text H^{n-2}(\alie ', M) & \text E^{n-1,0}_2 \, = \, H^{n-1}(\alie ', M) & \text H^n(\alie ', M) \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} \end{equation} \\

It follows that:
\begin{multline} \label{eq_Hineq}
\dim \Bigg[ \text H^{n-1} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \Bigg] \ - \ \dim \Bigg[ \text H^{n-2} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \Bigg] \\
\ \leq \ \dim \Big[ \text H^n(\alie, M) \Big] \ - \ \dim \Big[ \text H^n(\alie', M) \Big] \\
\leq \ \dim \Bigg[ \text H^{n-1} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \Bigg] \, . \quad
\end{multline}
Let us explain why. \\
%In \eqref{eq_spectralseq1} we see that the terms $E_2^{p,q}$, with $p \geq 0$ and $q \geq 2$, of the second sheet, are zero. It follows that the terms $E_r^{p,q}$, with $p \geq 0$ and $q \geq 2$, of the following sheets (i.e. for all $r \geq 2$) are also zero. Thus the terms $E_{\infty}^{p,q}$, with $p \geq 0$ and $q \geq 2$, of the limit sheet, are zero. \\
According to the bidegree $(2,-1)$ of the differentials in the second sheet \eqref{eq_2sheetspectralseq1}, it follows that the third sheet of the spectral sequence \eqref{eq_spectralseq1} for $N_1 = M$, centered at degree $n-1$, looks like:
\begin{equation} \label{eq_3sheetspectralseq1} \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text E^{n-2,1}_3 & \text E^{n-1,1}_3 \, = \, \text H^{n-1} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) & \text H^n \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \\
\text H^{n-2}(\alie ', M) & \text E^{n-1,0}_3 \, = \, H^{n-1}(\alie ', M) & \text E^{n,0}_3 \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} \end{equation}
$\text E^{n,0}_3$ is a quotient of $\text H^n(\alie ', M)$ by some image of $\text H^{n-2} \Big( \alie' \, , \, \text H^1(\ilie, M) \Big)$. Thus:
\begin{multline} \label{eq_dimE3}
\dim \Big[ \text H^n(\alie', M) \Big] \ - \ \dim \Bigg[ \text H^{n-2} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \Bigg]  \\
\leq \ \dim \text E^{n,0}_3 \ \leq \ \dim \Big[ \text H^n(\alie', M) \Big] \, .
\end{multline}
According to the bidegree $(r,1-r)$ of the differentials of sheet $r$ and from \eqref{eq_3sheetspectralseq1}, it follows that the spectral sequence degenerates at the third sheet. Thus, thanks to \eqref{eq_3sheetspectralseq1}, $\text H^n(\alie, M)$ has a filtration whose associated graded is linearly isomorphic to:
$$ \bigoplus_{p+q=n} \text E_3^{p,q} \ \simeq \ \text H^{n-1} \Big( \alie ' \, , \, \text H^1(\ilie, M) \Big) \, \oplus \, \text E_3^{n,0} \, . $$
Then \eqref{eq_Hineq} follows from \eqref{eq_dimE3}. \\

Let $N$ be a $\blie$-module. \\
Recall that, for all $p \in \NN$, there exists a linear isomorphism:
\begin{equation} \label{eq_ext}
\text H^p \Big( \blie \, , \, \text{Hom}_{\KK} (N,M) \Big) \ \simeq \ \text{Ext}^p_{\blie} (N,M) \, ;
\end{equation} \\

By restriction the $\blie$-module $M$ can be seen as an $(\alie')$-module, where the action of $\jlie$ is then trivial. \\
Thanks to \eqref{eq_NH0p}, \eqref{eq_NH1p}, \eqref{eq_NH2} and \eqref{eq_ext}, the second sheet of the spectral sequence \eqref{eq_spectralseq2} for $N_2 = M$, centered at degree $n-1$, looks like:
$$ \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text{Ext}^{n-2}_{\blie} (J, M) & \text F_2^{n-1,1} \, = \, \text{Ext}^{n-1}_{\blie} (J, M) & \text{Ext}^n_{\blie} (J, M) \\
\text H^{n-2}(\blie, M) & \text F_2^{n-1,0} \, = \, \text H^{n-1}(\blie, M) & \text H^n(\blie, M) \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} $$ \\

It follows that:
\begin{multline} \label{eq_Hineq2}
\dim \Big[ \text{Ext}_{\blie}^{n-1} (J,M) \Big] \ - \ \dim \Big[ \text{Ext}_{\blie}^{n-2} (J,M) \Big] \\
\ \leq \ \dim \Big[ \text H^n(\alie ', M) \Big] \ - \ \dim \Big[ \text H^n(\blie, M) \Big] \\
\leq \ \dim \Big[ \text{Ext}_{\blie}^{n-1} (J,M) \Big] \quad \, .
\end{multline}
The justifications of \eqref{eq_Hineq2} are similar to those of \eqref{eq_Hineq}. \\

Thanks to \eqref{eq_NH1} and \eqref{eq_NH1p}, one has the following linear isomorphisms (note that the actions of $\jlie$ on both $I$ and $M$, seen as $(\alie')$-modules, are trivial):
\begin{equation} \label{eq_HomS}
\text H^1 \Big( \jlie \, , \, \text H^1(\ilie, M) \Big) \ \simeq \ \text H^1 \Big( \jlie \, , \, \text{Hom}_{\KK}(I,M) \Big) \ \simeq \ \text{Hom}_{\KK} (T,M) \, .
\end{equation} \\

Let $m \in \ZZ$. Thanks to \eqref{eq_NH0p}, \eqref{eq_NH1p}, \eqref{eq_NH2}, \eqref{eq_ext} and  \eqref{eq_HomS}, the second sheet of the spectral sequence \eqref{eq_spectralseq2} for $N_2 = \text H^1(\ilie, M)$, centered at degree $m-1$, looks like:
$$ \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text{Ext}^{m-2}_{\blie} (T, M) & \text F_2^{n-1,1} \, = \, \text{Ext}^{m-1}_{\blie} (T, M) & \text{Ext}^m_{\blie} (T, M) \\
\text{Ext}^{m-2}_{\blie} (I, M) & \text F_2^{n-1,0} \, = \, \text{Ext}^{m-1}_{\blie} (I, M) & \text{Ext}^m_{\blie} (I, M) \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} $$ \\

It follows that:
\begin{multline} \label{eq_Hineq3}
\dim \Big[ \text{Ext}_{\blie}^{m-1} (T,M) \Big] \ - \ \dim \Big[ \text{Ext}_{\blie}^{m-2} (T,M) \Big] \\
\ \leq \ \dim \Bigg[ \text H^m \Big( \alie ', \text H^1(I,M) \Big) \Bigg] \ - \ \dim \Big[ \text{Ext}_{\blie}^m( I, M) \Big] \\
\leq \ \dim \Big[ \text{Ext}_{\blie}^{m-1} (T,M) \Big] \, . \quad
\end{multline}
The justifications of \eqref{eq_Hineq3} are similar to those of \eqref{eq_Hineq}. \\

One concludes by combining inequalities \eqref{eq_Hineq}, \eqref{eq_Hineq2} and \eqref{eq_Hineq3}.
\qed



\subsection{Kac-Moody algebras case} \label{subs_htilde}
We assume from here that the characteristic of $\KK$ is zero. \\

We apply results of \ref{subs_ablie} to the following situation: $\blie$ is a (non necessarely symmetrizable) Kac-Moody algebra which we rather denote by $\glie$, $\alie$ is the associated Kac-Moody algebra without Serre relations $\tglie$, $\ilie$ and $\jlie$ are the ideals $\tslie^-$ and $\tslie^+$ of respectively negative and positive Serre relations (see \ref{para_slie}). \\

Here, the $\blie$-modules $I$ and $J$ (they are defined in the beginning of \ref{subs_ablie} and they play a central role in proposition \ref{prop_ablie}) are respectively the $\glie$-modules $\tslie^- / [\tslie^-,\tslie^-]$ and $\tslie^+ / [\tslie^+,\tslie^+]$. We rather denote them respectively by $S^-$ and $S^+$. They are respectively called the negative Serre module and the positive Serre module. \\
Another $\blie$-module entered the game in \ref{subs_ablie}, namely $T = I \otimes_{\KK} J$. Here $T$ is the $\glie$-module $S^- \otimes_{\KK} S^+$, which is rather designated by $S$ and called the tensor Serre module. The Serre modules $S^-$, $S^+$ and $S$ will be studied in section \ref{sect_Serre}.

\begin{thm} \label{thm_htilde}
Let $M$ be a $\glie$-module and $n \in \NN$. Denote:
\begin{eqnarray*}
d_n &:= & \ \quad \dim \Big[ \text{Ext}_{\glie}^{\, n-1} (S^-, M) \Big] \ + \ \dim \Big[ \text{Ext}_{\glie}^{\, n-1} (S^+, M) \Big] \\
&& + \ \dim \Big[ \text{Ext}_{\glie}^{\, n-2} (S, M) \Big] \, ;
\end{eqnarray*}
\begin{eqnarray*}
d'_n &:= & \ \quad \dim \Big[ \text{Ext}_{\glie}^{\, n-2} (S^-, M) \Big] \ + \ \dim \Big[ \text{Ext}_{\glie}^{\, n-2} (S^+, M) \Big] \\
&& + \ \, 2 \: \! \dim \Big[ \text{Ext}_{\glie}^{\, n-3} (S, M) \Big] \, .
\end{eqnarray*}
The following inequality holds:
$$ d_n \ - \ d'_n \ \leq \ \dim \! \Big[ \text H^{\, n} (\tglie,M) \Big] \ - \ \dim \! \Big[ \text H^{ \, n} (\glie,M) \Big] \ \leq \ d_n \, . $$
\end{thm}

\proof
Recall paragraph \ref{para_slie}. \\
The Lie algebra $\glie$ is isomorphic to the Lie quotient of $\tglie$ by $\tslie = \tslie^- \oplus \tslie^+$. \\
Moreover $\tslie^{\pm}$ is a Lie subalgebra of the free Lie algebra $\tnlie^{\pm}$. According to the {\v{S}}ir{\v{s}}ov-Witt theorem (see \cite{Shi} and \cite{Wit}), $\tslie^{\pm}$ is also a free Lie algebra. \\
Since cohomological dimension of free Lie algebras are strictly less than $2$ (see for example \cite[corollary 7.2.5]{Wei}), one concludes thanks to proposition \ref{prop_ablie}.
\qed





\section{Serre Modules} \label{sect_Serre}
Theorem \ref{thm_htilde} involves the Serre modules $S^-$, $S^+$ and $S$ in order to compare the cohomologies of a Kac-Moody algebra $\glie$ and of the associated Kac-Moody algebra without Serre relations $\tglie$. We first prove that $S^-$ and $S^+$ are closely related thanks to the Cartan involution: see \ref{subs_SCartan}. We then study the structure of the negative Serre module $S^-$ and prove among others it belongs to the principal block of $\Owg$: see \ref{subs_negSerre}. \\

More precisely, theorem \ref{thm_htilde} relates cohomologies of $\glie$ and $\tglie$, with coefficients in a $\glie$-module $M$, in terms of the Ext groups $\text{Ext}_{\glie}^{\bullet}(S^-,M)$, $\text{Ext}_{\glie}^{\bullet}(S^+,M)$ and $\text{Ext}_{\glie}^{\bullet}(S,M)$. We prove in \ref{subs_extvanish} some vanishing results about these Ext groups. \\

The Kac-Moody algebra $\glie$ is assumed from now to be symmetrizable. Recall we assume the characteristic of $\KK$ is zero. \\

Denote by $\prs^{\pm}: \tslie^{\pm} \to S^{\pm}$ the natural projection and remark it is a morphism of $\tglie$-module.


\subsection{Cartan symmetry} \label{subs_SCartan}
We prove here that the Serre modules $S^-$ and $S^+$ are images of each other under the Cartan involution. This result will often allow us to restrict essentially our study to the case of $S^-$. \\

Recall that $\tilde \omega$ designates the Cartan involution of $\tglie$: see \ref{para_Cartaninv}. \\
Since $\tilde \omega$ is an automorphism of Lie algebra, one has:
$$ \tilde \omega (\tslie^{\pm}) \ = \ \tslie^{\mp} \, , \quad \quad \tilde \omega \Big( [\slie^{\pm},\slie^{\pm}] \Big) \ = \ [\slie^{\mp}, \slie^{\mp}] \, . $$
It follows that $\tilde \omega$ induces naturally a linear isomorphism:
$$ \omega_S^{\pm} \,: \ S^{\pm} \ \toiso \ S^{\mp} \, . $$

\begin{lem} \label{lem_SCartan}
The Cartan involution $\tilde \omega: \tglie \to \tglie$ induces an isomorphism of $\glie$-module:
$$  \omega_S^{\pm} \,: \ S^{\pm} \ \toiso \ (S^{\mp})^{\omega} \, . $$
\end{lem}

\proof
Let $v \in S^{\pm}$, $x \in \glie$ and $\tilde v \in \slie^{\pm}$, $\tilde x \in \tglie$ such that $\prg(\tilde x) = x$, $\prs^{\pm}(\tilde v) = v$ (see paragraph \ref{para_slie}). One has:
\begin{eqnarray*}
\omega_S^{\pm}(x.v) & = & \omega_S^{\pm} \Big( \prs^{\pm} \big( [\tilde x, \tilde v]_{\tglie} \big) \Big) \\
& = & \prs^{\mp} \Bigg( \tilde \omega \Big( [\tilde x, \tilde v]_{\tglie} \Big) \Bigg) \\
& = & \prs^{\mp} \Bigg( \Big[ \tilde \omega (\tilde x), \tilde \omega (\tilde v) \Big]_{\tglie} \Bigg) \\
& = & \big( \omega(x) \big) . \big( \omega^{\pm}_S (v) \big) \, .
\end{eqnarray*}
\qed



\subsection{Negative Serre module} \label{subs_negSerre}
We give here some description elements of the negative Serre module $S^-$. They are based on the following remark: $S^-$ is generated by the negative Serre relations (see \ref{para_slie}), which are highest weight vectors in $S^-$. Note analog results hold for $S^+$ (use for example the Cartan symmetry described in \ref{subs_SCartan}). \\

\begin{lem} \label{lem_negSerre}
\begin{enumerate}
\item[1)] $S^-$ is generated by the highest weight vectors $\text{pr}_S^-(u_{ij}^-)$ ($i, j \in I$, $i \neq j$).
\item[2)] One has the following exact sequence:
$$ \bigoplus_{i,j \in I, \, i \neq j} M \Big( - \alpha_j - (1 - a_{ij}) \alpha_i \Big) \ \to \ S^- \ \to \ 0 \, . $$
\item[3)] $\wt (S^-) \, \subset \ \bigcup_{i,j \in I, \, i \neq j} \, D \Big( - \alpha_j - (1 - a_{ij}) \alpha_i \Big)$.
\end{enumerate}
\end{lem}

\proof
\begin{enumerate}
\item[1)] The ideal $\tslie^-$ of $\tglie$ is generated by the negative Serre relations $u^-_{ij}$ ($i,j \in I$, $i \neq j$): see \ref{para_slie}.
In another hand, recall that one has in $\tglie$ (see again \ref{para_slie}):
$$ \Big[ e_k \, , \, u_{ij}^- \Big]_{\tglie} \ = \ 0 \, , \quad \ \forall \ i,j,k \in I, \ i \neq j \, . $$

In other words, the $\tglie$-module $\tslie^-$ (under the adjoint action) is generated by the highest weight vectors $u^-_{ij}$ ($i,j \in I$, $i \neq j$). One then concludes.
\item[2)] Fix $i, j \in I$ with $i \neq j$. In the $\tglie$-module $\tslie^-$, one has:
$$ \wt (u_{ij}^-) \ = \ - \alpha_j - (1 - a_{ij}) \alpha_i \, . $$
One then concludes.
\item[3)] Direct consequence of point 2.
\end{enumerate}
\qed \\

Recall the definition of the category $\Owg$ and of the principal block $\Owg_0$: see \ref{para_wg}.

\begin{cor} \label{cor_SOcat}
The negative Serre module $S^-$ belongs to the principal block $\Owg_0$ of $\Owg$.
\end{cor}

\proof
Fix $i, j \in I$ with $i \neq j$. One has:
$$ (s_i \: \! s_j) \ast 0 \ = \ s_i \big( s_j (\rho) \big) - \rho \ = \ s_i (\rho - \alpha_j) - \rho \ = \ - \alpha_j - (1 - a_{ij}) \alpha_i \, . $$
Thus $(- \alpha_j - (1 - a_{ij}) \alpha_i) \sim^W 0$. It follows that $M(- \alpha_j - (1 - a_{ij}) \alpha_i)$ is in $\Owg_0$. One then concludes thanks to point 2 of lemma \ref{lem_negSerre}.
\qed



\subsection{Ext vanishing results} \label{subs_extvanish}
We give some vanishing results about the Ext groups $\text{Ext}_{\glie}^{\bullet}(S^-,M)$, $\text{Ext}_{\glie}^{\bullet}(S^+,M)$ and $\text{Ext}_{\glie}^{\bullet}(S,M)$ when $M$ is in the category ${\mathcal O}$, or outisde the principal blocks ${\mathcal O}_0$ and $\Owg_0$. \\

The case of $S^-$ and $S^+$ are handled in \ref{para_extnegpos}. Note that, when $\glie$ is infinite-dimensional, the situations of $S^-$ and $S^+$ are seemingly different. One cannot use here the Cartan symmetry described in \ref{subs_SCartan}. The case of the tensor Serre module is handled in \ref{para_exttensor}. It needs more work and use several intermediate technical results, which we have postponed in an appendix (see section \ref{sect_appendix}). \\

We prove here:
\begin{enumerate}
\item[\textbullet] $\text{Ext}_{\glie}^{\bullet}(S^-,M) = \text{Ext}_{\glie}^{\bullet}(M,S^-) = 0$, for all $M$ outside the principal blocks: see proposition \ref{prop_extneg};
\item[\textbullet] when $\glie$ is finite-dimensional, $\text{Ext}_{\glie}^{\bullet}(S^+,M) = \text{Ext}_{\glie}^{\bullet}(M,S^+) = 0$, for all $M$ outside the principal blocks: see proposition \ref{prop_extpos};
\item[\textbullet] $\text{Ext}_{\glie}^0(S^+,M) = 0$, for all $M$ in ${\mathcal O}$: see lemma \ref{lem_extpos};
\item[\textbullet] $\text{Ext}_{\glie}^0(S,M) = \text{Ext}_{\glie}^0(M,S) = 0$, for all $M$ in ${\mathcal O}$: see theorem \ref{thm_ext0S}.
\end{enumerate}


\subsubsection{} \label{para_extnegpos}
\begin{prop} \label{prop_extneg}
For all $M$ in ${\mathcal O}_{\Lambda}$ or $\Owg_{\Lambda^0}$ with $\Lambda, \Lambda^0 \neq 0$, the following holds:
$$ \text{Ext}_{\glie}^{\, \bullet} (S^-,M) \ = \ \text{Ext}_{\glie}^{\, \bullet} (M,S^-) \ = \ 0 \, . $$
\end{prop}

\proof
Since $S^-$ is in $\Owg_0$ thanks to corollary \ref{cor_SOcat}, the proposition is a consequence of \cite[theorem 3.3.8]{KumBook}.
\qed \\

\begin{prop} \label{prop_extpos}
Suppose that $\glie$ is finite-dimensional. \\
For all $M$ in ${\mathcal O}_{\Lambda}$ with $\Lambda \neq 0$, the following holds:
$$ \text{Ext}_{\glie}^{\, \bullet} (S^+,M) \ = \ \text{Ext}_{\glie}^{\, \bullet} (M,S^+) \ = \ 0 \, . $$
\end{prop}

\proof
The Serre module $S^-$ belongs to the principal block ${\mathcal O}_0$: see corollary \ref{cor_SOcat}. Thus $Z_U(\glie)$ acts on $S^-$ by the central character $0 \circ \mathcal H$. Thanks to lemma \ref{lem_SCartan}, it follows that $Z_U(\glie)$ also acts on $S^+$ by the central character $0 \circ \mathcal H$. \\
In another hand, since $\lambda \sim^W 0 \Leftrightarrow (\lambda \circ \mathcal H) = 0$ (see paragraph \ref{para_wg}), the actions of $Z_U(\glie)$ on $S^+$ and $M$ differ. One then concludes.
\qed \\

\begin{remT}
Following lemma \ref{lem_extpos} and proposition \ref{prop_Sint} can be skipped in the way to theorem \ref{thm_swhlemma}.
\end{remT}

\begin{lem} \label{lem_extpos}
For all $M$ in the category ${\mathcal O}$, the following holds:
$$ \text{Ext}_{\glie}^{\, 0}(S^+,M) \ = \ 0 \, . $$
\end{lem}

\proof
Let $M$ in ${\mathcal O}$. Thanks to lemma \ref{lem_finiteseq}, one can suppose without loss of generality that either $M$ is simple or $\wt M \cap D^{\geq}(0)$ is empty.
\begin{enumerate}
\item[a)] Suppose that $M$ is simple. Using Cartan symmetry \ref{lem_SCartan}, it is equivalent to prove that $\text{Ext}^0_{\glie}(S^-,M^{\omega})$ vanishes. Suppose there exists a nonzero morphism from $S^-$ to $M^{\omega}$ and denote $\mu_{ij}^- := - \alpha_j - (1 - a_{ij}) \alpha_i$. In view of point 2 of lemma \ref{lem_negSerre}, there exist $i,j \in I$ with $i \neq j$ and a nonzero morphism from $M(\mu_{ij}^-)$ to $M$. This imply that $L(\mu_{ij}^-)$ is isomorphic to $M^{\omega}$ since $M^{\omega}$ is simple. Besides, the actions of $e_i$ and $f_i$ ($i \in I$) are locally nilpotent on respectively $L(\mu_{ij}^-)$ and $M^{\omega}$, since $L(\mu_{ij}^-)$ and $M$ are in ${\mathcal O}$. Thus $L(\mu_{ij}^-)$ is integrable and $\mu_{ij}^-$ dominant. This is impossible since:
$$ \alpha_i^{\vee} \big( \mu_{ij}^- \big) \ = \ a_{ij} - 2 \ \leq \ -2 \, . $$
\item[b)] Suppose that $\wt (M) \cap D^{\geq}(0)$ is empty. In view of point 3 of lemma \ref{lem_negSerre} and using the Cartan symmetry \ref{lem_SCartan}, $\wt (M) \cap \wt (S^+)$ is then also empty. One concludes.
\end{enumerate}
\qed \\

\begin{prop} \label{prop_Sint}
Let $M$ be an integrable $\glie$-module. The following holds:
$$ \text{Ext}^{\, 0}_{\glie}(S^-,M) \ = \ \text{Ext}^{\, 0}_{\glie}(S^+,M) \ = \ 0 \, . $$
\end{prop}

\proof
Consequence of theorem \ref{thm_htilde} and remark \ref{rem_coho1}.
\qed

\begin{remmm}
One can give a more direct proof of proposition \ref{prop_Sint}. \\
Suppose there exists a nonzero morphism from $S^-$ to $M$. Then, in view of point 2 of lemma \ref{lem_negSerre}, there exist $i,j \in I$ with $i \neq j$ and a nonzero morphism from $M(- \alpha_j - (1 - a_{ij}) \alpha_i)$ to $M$. This implies that $L(- \alpha_j - (1 - a_{ij}) \alpha_i)$ is integrable and that $(- \alpha_j - (1 - a_{ij}) \alpha_i)$ is dominant. This is impossible since:
$$ \alpha_i^{\vee} \big( \mu_{ij}^- \big) \ = \ a_{ij} - 2 \ \leq \ -2 \, . $$
The case of $S^+$ follows from Cartan symmetry \ref{lem_SCartan} and from the fact that $M^{\omega}$ is still integrable. \\
The author believes it is possible to prove the following when $M$ is again integrable:
$$ \text{Ext}^{\, 0}_{\glie}(M,S^-) \ = \ \text{Ext}^{\, 0}_{\glie}(M,S^+) \ = \ 0 \, . $$
\end{remmm}


\subsubsection{} \label{para_exttensor}
\begin{thm} \label{thm_ext0S}
For all $M$ in the category ${\mathcal O}$, the following holds:
$$ \text{Ext}^{\, 0}_{\glie} (S,M) \ = \ \text{Ext}^{\, 0}_{\glie} (M,S) \ = \ 0 \, . $$
\end{thm}

\begin{remT}
The long proof below of theorem \ref{thm_ext0S} can be drastically shortened if one is only interested in proving that $\text{Ext}^{\, 0}_{\glie} (S,M)$ vanishes for a simple $\glie$-module $M \neq \KK$ in ${\mathcal O^{\mathrm{int}}}$. In this case, just use point 2-b of the proof below and lemma \ref{lem_dominant}.
\end{remT}

\begin{rem} \label{rem_ext0Sproof}
Let us explain the idea of the proof of theorem \ref{thm_ext0S}. \\
We first reduce the problem to the following one:
$$ \text{Ext}^{\, 0}_{\blie^-} (S,\KK_{\lambda}) \ = \ \text{Ext}^{\, 0}_{\blie^-} (\KK_{\lambda},S) \ = \ 0 \, , \quad \ \lambda \in \hlie^{\ast} \, . $$
The latter is handled in the appendix: see proposition \ref{prop_STHom}. However, the cases where $\lambda \in A$ cannot be solved by this method. Note that, in the fast way to theorem \ref{thm_swhlemma}, these cases appeared irrelevant: see lemma \ref{lem_dominant}. Let us now describe how they are tackled in the full proof of theorem \ref{thm_ext0S}. \\
Suppose that $\lambda \in A$. The simple module $M = L(\lambda)$ actually satisfies the particular conditions of point 2 of proposition \ref{prop_gleqdimext}. This allows us to prove that $\text H^{\, 2}(\tglie,M)$ is isomorphic to $\text H^{\, 2}(\tglie / \slie^+,M)$. Using Hochschild-Serre spectral sequence and the fact that $\slie^+$ is a free Lie algebra (see the proof of theorem \ref{thm_htilde}), we prove (in a similar way than the one used for proposition \ref{prop_ablie}):
\begin{equation} \label{eq_ext0Sproof}
\text H^{\, 2}(\tglie,M) \ \simeq \ \text H^{\, 2}(\glie,M) \, \oplus \, \text{Ext}_{\glie}^{\, 1} (S^-,M) \, \oplus \, \text{Ext}_{\glie}^{\, 1} (S^+,M) \, .
\end{equation}
In another hand, theorem \ref{thm_htilde} provides the same kind of result. We prove the only difference is the appearance of $\text{Ext}_{\glie}^{\, 0}(S,M)$ in the right hand side of \eqref{eq_ext0Sproof}. Modulo some finite-dimensional remarks, it then follows that $\text{Ext}_{\glie}^{\, 0}(S,M)$ has to vanish.
\end{rem}

\proof
\begin{enumerate}
\item[1)] Let $M$ in ${\mathcal O}$, we first prove that $\text{Ext}^0_{\glie} (M,S)$ vanishes. \\
Thanks to lemma \ref{lem_hwseq}, one can without loss of generality suppose that $M$ is a highest weight module. Denote by $v$ a highest weight vector of $M$ and let $f \in \text{Hom}_{\glie}(M,S)$. \\
Since $v$ is a highest weight vector, $\KK . v$ is a $(\blie^+)$-submodule of $M$. Thanks to lemma \ref{lem_SCartan} and point 1 of proposition \ref{prop_STHom}, the restriction of $f$ to $\KK . v$ is thus zero. In another hand, $M$ is generated as a $\glie$-module by $v$. As a consequence, $f$ is zero.
\item[2)] Denote:
$$ A \ := \ \Big \{ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, ; \ \ i,j,k,l \in I, \ i \neq j, \, k \neq l \Big \} \, . $$
Let $M$ in ${\mathcal O}$, we prove here that $\text{Ext}^0_{\glie} (S,M)$ vanishes. \\
Suppose there exists a nonzero $f \in \text{Hom}_{\glie}(S,M)$. Without loss of generality, one can suppose that $f$ is surjective. \\
Let $\lambda_m \in \hlie^{\ast}$ such that $A \subset D^{\geq}(\lambda_m)$. Thanks to lemma \ref{lem_finiteseq}, one can thus suppose that $M$ is simple or that $\wt M \cap A = \emptyset$.
\begin{enumerate}
\item[a)] Suppose that $\wt M \cap A = \emptyset$. \\
Since $M$ is in ${\mathcal O}$, there exists a maximal weight $\lambda$ among $\wt M$. Thus $M':= \bigoplus_{\mu \neq \lambda} M_{\mu}$ is a $(\blie^-)$-submodule of $M$. Since $f$ is surjective, it induces a nonzero morphism of $(\blie^-)$-module from $S$ to $\KK_{\lambda} \simeq M / M'$. In view of point 2 of proposition \ref{prop_STHom} and since $\lambda \notin A$, there is a contradiction.
\item[b)] Suppose that $M = L(\lambda)$ with $\lambda \notin A$. \\
$M':= \bigoplus_{\mu < \lambda} M_{\mu}$ is a $(\blie^-)$-submodule of $M$. Since $f$ is surjective, it induces a nonzero morphism of $(\blie^-)$-module from $S$ to $\KK_{\lambda} \simeq M / M'$. In view of point 2 of proposition \ref{prop_STHom} and since $\lambda \notin A$, there is a contradiction.
\item[c)] Suppose that $M = L(\lambda)$ with $\lambda \in A$. \\
Denote: $\tglie^+ := \tglie / \tslie^+$. Thanks to \eqref{eq_ADg} and point 3 of proposition \ref{prop_gleqdimext}, one has:
$$ \text{YExt}_{\tglie}^1(\tglie,M) \ \simeq \ \text{YExt}_{\tglie^+}^1(\tglie^+,M) \, . $$
In another hand, it is known (see for example \cite[theorem 7.6.3]{Wei}) that vector spaces $\text H^2(\alie,N)$ and $\text{Ext}_{\alie}^1(\alie,N)$ are isomorphic ($\alie$ is a Lie algebra, seen as a $\alie$-module with respect to the adjoint action, $N$ is a $\alie$-module). Thus:
\begin{equation} \label{eq_h2gp}
\text H^2(\tglie,M) \ \simeq \ \text H^2(\tglie^+,M) \, .
\end{equation}
By abuse of notation, $\tslie^-$ will also designate the ideal $\tslie / \tslie^+$ of $\tglie^+$. There is natural identification between the Lie algebras $\glie$ and $\tglie^+ / \tslie^-$. Consider the (convergent) Hochschild-Serre spectral sequence (see \cite{HS}):
\begin{equation} \label{eq_spectralgp}
\text E^2_{p,q} \ = \ \text H^p \Big( \glie \, , \, \text H^q(\tslie^-, M) \Big) \ \Rightarrow \ \text H^{p+q}(\tglie^+,M) \, .
\end{equation}
Since the induced action of $\tslie^-$ on $M$ is trivial, there exist isomorphisms of $\glie$-module:
\begin{equation} \label{eq_MH01}
\text H^0(\tslie^-, M) \ \simeq \ M \, , \quad \ \text H^1(\tslie^-, M) \ \simeq \ \text{Hom}_{\KK}(S^-, M) \, .
\end{equation}
Recall the cohomological dimension of $\tslie^-$ is strictly less than 2: see the proof of theorem \ref{thm_htilde}. Since the induced action of $\tslie^-$ on $M$ is trivial, one thus has:
\begin{equation} \label{eq_MH2}
\text H^q(\tslie^-, M) \ = \ 0 \, , \quad \ \forall \ q \geq 2 \, .
\end{equation}
Recall that, for all $p \in \NN$, there exists a linear isomorphism:
\begin{equation} \label{eq_extglie}
\text H^p \Big( \glie \, , \, \text{Hom}_{\KK} (S^-,M) \Big) \ \simeq \ \text{Ext}^p_{\glie} (S^-,M) \, .
\end{equation} \\
Thanks to \eqref{eq_MH01}, \eqref{eq_MH2} and \eqref{eq_extglie}, the second sheet of the spectral sequence \eqref{eq_spectralgp}, centered at degree $1$, looks like:
\begin{equation} \label{eq_2sheetspectralgp} \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text{Ext}^0_{\glie} (S^-, M) & \text E^{1,1}_2 \, = \, \text{Ext}^1_{\glie} (S^-, M) & \text{Ext}^2_{\glie} (S^-, M) \\
\text H^0(\glie, M) & \text E^{1,0}_2 \, = \, \text H^1(\glie, M) & \text H^2(\glie, M) \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} \end{equation}
It follows that:
\begin{multline} \label{eq_Hineqgp}
\dim \Big[ \text{Ext}^1_{\glie} (S^-,M) \Big] \ - \ \dim \Big[ \text{Ext}^0_{\glie} (S^-,M) \Big] \\
\ \leq \ \dim \Big[ \text H^2(\tglie^+, M) \Big] \ - \ \dim \Big[ \text H^2(\glie, M) \Big] \\
\leq \ \dim \Big[ \text{Ext}^1_{\glie} (S^-,M) \Big] \, . \quad
\end{multline}
Thanks to lemma \ref{lem_extSA}, one thus has:
\begin{equation} \label{eq_h2ggp}
\text H^2(\tglie^+,M) \ \simeq \ \text H^2(\glie,M) \, \oplus \, \text{Ext}_{\glie}^1(S^-,M) \, .
\end{equation}
Let us explain inequality \eqref{eq_Hineqgp}. \\
According to the bidegree $(2,-1)$ of the differentials in the second sheet \eqref{eq_2sheetspectralgp}, it follows that the third sheet of the spectral sequence \eqref{eq_spectralgp}, centered at degree $1$, looks like:
\begin{equation} \label{eq_3sheetspectralgp} \xymatrix @R=1pc @C=1.2pc {
\vdots & \vdots & \vdots \\
0 & 0 & 0 \\
\text{Ext}^0_{\glie} (S^-, M) & \text E^{1,1}_3 \, = \, \text{Ext}^1_{\glie} (S^-, M) & \text{Ext}^2_{\glie} (S^-, M) \\
\text H^0(\glie, M) & \text E^{1,0}_3 \, = \, H^1(\glie, M) & \text E^{2,0}_3 \\
0 & 0 & 0 \\
\vdots & \vdots & \vdots
} \end{equation}
$\text E^{2,0}_3$ is a quotient of $\text H^2(\glie, M)$ by some image of $\text{Ext}^0_{\glie} (S^-, M)$. Thus:
\begin{multline} \label{eq_dimE3gp}
\dim \Big[ \text H^2(\glie, M) \Big] \ - \ \dim \Big[ \text{Ext}^0_{\glie} (S^-, M) \Big] \\
\leq \ \dim \text E^{2,0}_3 \ \leq \ \dim \Big[ \text H^2(\glie, M) \Big] \, .
\end{multline}
According to the bidegree $(r,1-r)$ of the differentials of sheet $r$ and from \eqref{eq_3sheetspectralgp}, it follows the spectral sequence degenerates at the third sheet. Thus, thanks to \eqref{eq_3sheetspectralgp}, $\text H^n(\alie, M)$ has a filtration whose associated graded is linearly isomorphic to:
$$ \text E_3^{0,2} \, \oplus \, \text E_3^{1,1} \, \oplus \, \text E_3^{2,0} \ \simeq \ \text{Ext}^1_{\glie} (S^-, M) \, \oplus \, \text E_3^{2,0} \, . $$
Then \eqref{eq_Hineqgp} follows from \eqref{eq_dimE3gp}. \\
Let us summarize: combining \eqref{eq_h2gp} and \eqref{eq_h2ggp}, the following holds:
\begin{equation} \label{eq_h2gggp}
\text H^2(\tglie,M) \ \simeq \ \text H^2(\glie,M) \, \oplus \, \text{Ext}_{\glie}^1(S^-,M) \, .
\end{equation}
We have then established some connection between the cohomologies of $\glie$ and $\tglie$. This is exactly the topic, which theorem \ref{thm_htilde} deals with. More precisely, thanks to lemma \ref{lem_extpos} and \ref{lem_extSA}, theorem \ref{thm_htilde} implies:
\begin{equation} \label{eq_h2htilde}
\text H^2(\tglie,M) \ \simeq \ \text H^2(\glie,M) \, \oplus \, \text{Ext}_{\glie}^1(S^-,M) \, \oplus \,  \text{Ext}_{\glie}^0(S,M) \, .
\end{equation}
Since $\text H^2(\glie,M)$ and $\text{Ext}_{\glie}^1(S^-,M)$ are finite-dimensional (see just below), from \eqref{eq_h2gggp} and \eqref{eq_h2htilde} one can conclude: $\text{Ext}_{\glie}^0(S,M) = 0$. \\

Let $X$ be a $\glie$-module in ${\mathcal O}$ and let $n \in \NN^{\ast}$, a Verma finite $n$-resolution of $X$ is a short exact sequence
$$ X_n \ \to \ X_{n-1} \ \to \ \cdots \ \to \ X_1 \ \to \ X \ \to \ 0 \, , $$
such that, for all $1 \leq k \leq n$, $X_k$ is a finite direct sum of Verma modules. By convention, $X$ always has a Verma finite $0$-resolution. We say that $X$ has a Verma finite $\infty$-resolution if $X$ has a Verma finite $n$-resolution for all $n \in \NN$. Denote:
$$ \Vf (X) \ := \ \text{max} \Big\{ n \in \NN \cup \{ \infty \} \, , \ \text{$X$ has a Verma finite $n$-resolution} \Big \} \, . $$
Let us prove by induction that, for all $n \in \NN$ and for all $\glie$-modules $X,Y$ in ${\mathcal O}$, $\text{Ext}^n_{\glie}(X,Y^{\vee})$ is finite-dimensional if $\Vf (X) \geq n+1$ and $\Vf (Y) \geq n$. \\
Let us consider the case $n=0$. Since $\Vf (X) \geq 1$, $X$ is finitely generated by weight vectors. Moreover, since a morphism of $\glie$-module from $X$ to $Y^{\vee}$ is uniquely specified by its values on the generating weight vectors and since the weight spaces of $Y^{\vee}$ are finite-dimensional, it follows that $\text{Ext}^0_{\glie}(X,Y^{\vee})$ is finite-dimensional. \\
Fix $n \in \NN^{\ast}$ and assume by induction that the assertion is true at rank $n-1$. We have the following exact sequence:
$$ \text{Ext}^{n-1}_{\glie}(X'_1,Y^{\vee}) \ \to \ \text{Ext}^n_{\glie}(X,Y^{\vee}) \ \to \ \text{Ext}^n_{\glie}(X_1,Y^{\vee}) \, , $$
where $X_1$ is the first component of a Verma finite $(n+1)$-resolution of $X$ and where $X_1'$ is the kernel of the corresponding surjective morphism $X_1 \to X$. By induction hypothesis (remark that $\Vf (X'_1) \geq n$), it is then sufficient to prove that $\text{Ext}^n_{\glie}(X,Y^{\vee})$ is finite-dimensional, when $X$ is a Verma module. Thus suppose that $X$ is a Verma module from now. \\
We have the following exact sequence:
$$ \text{Ext}^{n-1}_{\glie}(X,(Y'_1)^{\vee}) \ \to \ \text{Ext}^n_{\glie}(X,Y^{\vee}) \ \to \ \text{Ext}^n_{\glie}(X,(Y_1)^{\vee}) \, , $$
where $Y_1$ is the first component of a Verma finite $n$-resolution of $Y$ and where $Y_1'$ is the kernel of the corresponding surjective morphism $Y_1 \to Y$. Since $X$ is a Verma module, $\Vf (X) = \infty$. Thus, by induction hypothesis ($\Vf (Y_1') \geq n-1$), it is sufficient to prove that $\text{Ext}^n_{\glie}(X,Y^{\vee})$ is finite-dimensional, when $Y$ is also a Verma module. \\
Let $\mu, \nu \in \hlie^{\ast}$ such that $X = M(\mu)$ and $Y = M(\nu)$. Using results of \cite{KumBook}, one has:
$$ \text{Ext}^n_{\glie}(X,Y^{\vee}) \ \simeq \ \Big( \text{Tor}_n^{\glie}((X^{\omega})^t,Y) \Big)^{\ast} \, ; \quad \ \text{\cite[lemma 3.3.5]{KumBook}} $$
\begin{eqnarray*}
\text{Tor}_n^{\glie}((X^{\omega})^t,Y) & \simeq & \text{Tor}^{\blie^+}_n((X^{\omega})^t,\KK_{\nu}) \, , \quad \ \text{\cite[lemma 3.1.14]{KumBook}} \\
& \simeq & \text{Tor}^{\blie^+}_n (\KK_{\nu}^t, X^{\omega}) \, , \quad \ \text{\cite[lemma 3.1.13]{KumBook}} \\
& \simeq & \text{Tor}^{\hlie}_n (\KK_{\nu}^t, \KK_{- \mu}) \, , \quad \ \text{\cite[lemma 3.1.14]{KumBook}} \\
& \simeq & \text H_n (\hlie,\KK_{\nu-\mu}) \, , \quad \ \text{\cite[lemmas 3.1.9 \& 3.1.13]{KumBook}}
\end{eqnarray*}
where $N^{\: \! t}$ designates the right $\glie$-module built from a left $\glie$-module $N$ by the twist $(- \text{id}_{\glie})$. Recall also the definition of the $(\blie^-)$-module $\KK_{\mu}$ given in \ref{app_tensor}. The definition for $(\blie^+)$ is similar. \\
The Lie algebra $\hlie$ is finite-dimensional, and so is the $\hlie$-module $\KK_{\nu - \mu}$. It follows that $H_n (\hlie,\KK_{\nu-\mu})$ is finite-dimensional. This ends the induction proof. \\

Point 2 of lemma \ref{lem_negSerre} implies: $\Vf (S^-) \geq 1$. Since $M$ is simple, one has: $\Vf (M) \geq 1$. Besides, $\text H^2(\glie,M) \simeq \text{Ext}^2_{\glie}(\KK,M)$ and $\Vf (\KK) \geq 2$ since there is a natural exact Verma finite $2$-resolution of $\KK$:
$$ \bigoplus_{i \in I} \, M(-\alpha_i) \ \to \ M(0) \ \to \ \KK \ \to \ 0 \, . $$
One can conclude: $\text{Ext}^1_{\glie} (S^-,M)$ and $\text H^2(\glie,M)$ are finite-dimensional.
\end{enumerate}
%Since ${\mathcal O^{\mathrm{int}}}$ is completely reducible, one can suppose that $M = L(\lambda)$ with $\lambda$ dominant. One has to distinguish two cases.
%\begin{enumerate}
%\item[a)] $\lambda \neq 0$. Then, thanks to lemma \ref{lem_dominant}, $\lambda \notin A$ and one concludes thanks to point 3) a).
%\item[b)] $\lambda = 0$. \\
%It is known (see for example \cite{Wei}) that vector spaces $\text H^2(\alie,N)$ and $\text{Ext}_{\alie}^1(\alie,N)$ are isomorphic ($\alie$ is a Lie algebra, seen as a $\alie$-module with respect to the adjoint action, $N$ is a $\alie$-module). Thus, thanks to lemma \ref{lem_gleqdimext} and lemma \ref{lem_AD0}, one has:
%$$ \dim \Bigg[ \text H^2 \Big( \tglie, \KK \Big) \Bigg] \ = \ \dim \Bigg[ \text H^2 \Big( \glie, \KK \Big) \Bigg] \, . $$
%Thus, thanks to Cartan symmetry \ref{lem_SCartan}, lemma \ref{lem_SExt}, lemma \ref{lem_AD0}, and theorem \ref{thm_htilde}, one has $\text{Ext}^0_{\glie} (S,M) = 0$.
%\end{enumerate}
\end{enumerate}
\qed

\begin{remmm}
The author believes the proof of theorem \ref{thm_ext0S} can be shortened. Indeed it could be possible (when $\glie$ is finite-dimensional, it is a certainty) that $\text{Ext}^{\, 1}_{\glie} (S^-,M)$ and $\text H^{\, 2}(\glie,M)$ actually vanish when $M = L(\lambda)$ whith $\lambda \in A$ (see the proof of the theorem for the definition of $A$). The arguments should be more consice that the ones used to prove that $\text{Ext}^{\, 1}_{\glie} (S^-,M)$ and $\text H^{\, 2}(\glie,M)$ are finite-dimensional.
\end{remmm}





\section{Cohomology of Kac-Moody Algebras Without Serre Relations} \label{sect_KWS}
The previous two sections \ref{sect_ablie} and \ref{sect_Serre} are applied in order to obtain the main results of this part. The strategy is simple: thanks to theorem \ref{thm_htilde}, we calculate some cohomologies of a Kac-Moody algebra without Serre relations $\tglie$, from known cohomologies of the associated Kac-Moody algebra with Serre relations $\glie$, by using the Ext vanishing results established in \ref{subs_extvanish}. \\

Here are the results of this section.
\begin{enumerate}
\item[\textbullet] We prove the second cohomology group $\text H^2(\tglie)$ is isomorphic to the second cohomology group $\text H^2(\glie)$. See theorem \ref{thm_coho2}.
\item[\textbullet] Let $M$ be a $\glie$-module in ${\mathcal O}$, outside the principal blocks. We prove that $\text H^1(\tglie,M)$ vanishes. When $\glie$ is finite-dimensional, we prove that $\text H^2(\tglie,M)$ also vanishes. When $\glie$ is infinite-dimensional, we prove that $\text H^2(\tglie,M)$ is isomorphic to $\text{Ext}^1_{\glie}(S^+,M)$. See theorems \ref{thm_h1kac}, \ref{thm_h2} and proposition \ref{prop_h2kac}. It is conjectured in \ref{subs_further} that the latter actually vanishes: see conjectures \ref{conj_extpos} and \ref{conj_h2kac}. \\
These results have to compared with known ones about the cohomology of $\glie$: $\text H^{\bullet}(\glie,M) = 0$. When $\glie$ is finite-dimensional, it is a consequence of the separation of the Weyl orbits by the center of $U(\glie)$. For a general Kac-Moody algebra, Kumar proved it for the category ${\mathcal O}$ and the subcategory $\Owg$: see \cite[corollary 3.3.10.b2]{KumBook}.
\item[\textbullet] We establish the originally wanted result of this part, i.e. the free Serre relations version of second Whitehead's lemma: $\text H^2(\tglie,M) = 0$ for all finite-dimensional $\tglie$-modules, when $\glie$ is finite-dimensional. See theorem \ref{thm_swhlemma}. \\
As already said, the free Serre relations version of first Whitehead's lemma also holds and the proof is quite straightforward: see remark \ref{rem_fsrvwl1}.
\end{enumerate}

\begin{remT}
Recall the original motivation of this part was the free Serre relations version of second Whitehead's lemma, which appears as a direct consequence of theorems \ref{thm_coho2} and \ref{thm_h2}. As already mentioned one can give a shorter and more natural proof of it. This one is divided into two parts. We indeed distinguish between the case of the trivial $\tglie$-module $\KK$ and the case of a finite-dimensional and simple $\tglie$-module $M \neq \KK$. Note this kind of distinction is often made in the proof of usual second Whitehead's lemma. The case of $\KK$ is directly handed through some related first (Yoneda) extension groups: see \ref{app_ext} with corollary \ref{cor_gleqdimext} and the second proof of theorem \ref{thm_coho2}. For the second case, we use a simplified version of theorem \ref{thm_h2}: when $\glie$ is finite-dimensional, $\text H^{\, 2}(\tglie,M)$ vanishes for all finite-dimensional simple $\glie$-modules $M \neq \KK$. The strategy to prove it is the same than the one explained just above, but one only needs a simplified version of theorem \ref{thm_ext0S} (see the remark ``Towards" which goes with the theorem).
\end{remT}

In this section, unless explicitly stated, $\glie$ designates a (symmetrizable) Kac-Moody algebra. We recall the characteristic of $\KK$ is assumed to be zero.


\subsection{Second cohomology group} \label{subs_coho2}
We prove here the second cohomology group $\text H^2(\tglie)$ of a Kac-Moody algebra without Serre relations $\tglie$ is isomorphic to the second cohomology group $\text H^2(\glie)$ of the associated Kac-Moody algebra with Serre relations $\glie$. We remark the same holds for the first cohomology group $\text H^1(\tglie)$. \\

\begin{thm} \label{thm_coho2}
The second cohomology groups of $\glie$ and $\tglie$ are isomorphic:
$$ \text H^{\, 2}(\tglie) \ \simeq \ \text H^{\, 2} (\glie) \, . $$
\end{thm}

\begin{remT}
If one has chosen to follow the fast way to theorem \ref{thm_swhlemma}, only the second proof below of theorem \ref{thm_coho2} has to be considered.
\end{remT}

\proof
We give two different proofs of the theorem. \\
Recall that $\text H^2(\tglie):= \text H^2(\tglie,\KK)$.
\begin{enumerate}
\item[1)] Consequence of theorem \ref{thm_htilde}, theorem \ref{thm_ext0S} and corollary \ref{cor_SExt}.
\item[2)] It is known (see for example \cite[theorem 7.6.3]{Wei}) that vector spaces $\text H^2(\alie,N)$ and $\text{Ext}_{\alie}^1(\alie,N)$ are isomorphic ($\alie$ is a Lie algebra, seen as a $\alie$-module with respect to the adjoint action, $N$ is a $\alie$-module). Thus, thanks to corollary \ref{cor_gleqdimext}, one has ($\KK$ is seen as an invariant $\glie$-module):
$$ \text H^2( \tglie, \KK) \ \simeq \ \text H^2( \glie, \KK) \, . $$
\end{enumerate}
\qed \\

\begin{remmm}
The second proof of theorem \ref{thm_coho2} is independent from theorem \ref{thm_ext0S}. It can be used to obtain a shorter proof of $\text{Ext}_{\glie}^{\, 0}(S, \KK) = 0$, than the one given by long point 2-c in the proof of theorem \ref{thm_ext0S}.
\end{remmm}

\begin{rem} \label{rem_coho1}
The first cohomology groups $\text H^{\, 1}(\glie)$ and $\text H^{\, 1}(\tglie)$ of $\glie$ and $\tglie$ are also isomorphic. \\
More generally, the cohomologies of $\glie$ and $\tglie$ with coefficients in any integrable $\glie$-module are isomorphic. The proof is quite straightforward thanks to lemma \ref{lem_Ytglie} and the following fact (see \cite[corollary 7.3.6]{Wei}):
$$ \text H^{\, \bullet} (\alie,N) \ \simeq \ \text{Ext}_{\alie}^{\, \bullet}(\KK,N) \quad \ \text{($\alie$ is a Lie algebra, M,N are $\alie$-modules)} \, . $$
\end{rem}

\begin{remmm}
There is no reason that the same phenomenon still occurs for higher cohomology groups. At this matter, see remark \ref{rem_end}.
\end{remmm}



\subsection{Cohomology outside the principal blocks} \label{subs_principalblock}
We describe here the cohomologies $\text H^1(\tglie,M)$ and $\text H^2(\tglie,M)$ of a Kac-Moody algebra without Serre relations $\tglie$, with coefficients in a $\glie$-module $M$ outside the principal blocks. We prove that $\text H^1(\tglie,M)$ vanishes. When $\glie$ is finite-dimensional, we prove that $\text H^2(\tglie,M)$ also vanishes. When $\glie$ is infinite-dimensional, we prove that $\text H^2(\tglie,M)$ is isomorphic to $\text{Ext}^1_{\glie}(S^+,M)$. It is conjectured in \ref{subs_further} that the latter actually vanishes: see conjectures \ref{conj_extpos} and \ref{conj_h2kac}. \\
Note that, in the case $\glie$, one has: $\text H^{\bullet}(\glie,M) = 0$ (see \cite[corollary 3.3.10.b2]{KumBook}). \\

\begin{remT}
Theorem \ref{thm_h1kac} can be skipped in the way to theorem \ref{thm_swhlemma}. If one has considered the proof of theorem \ref{thm_ext0S} in the case of a simple $\glie$-module $M \neq \KK$ in ${\mathcal O^{\mathrm{int}}}$, the statements of proposition \ref{prop_h2kac} and theorem \ref{thm_h2} have to be modified accordingly.
\end{remT}

\begin{thm} \label{thm_h1kac}
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ or in $\Owg_{\Lambda^0}$, with $\Lambda, \Lambda^0 \neq 0$. \\
The following holds:
$$ \text H^{\, 1}(\tglie,M) \ \simeq \ 0 \, . $$
\end{thm}

\proof
Consequence of theorem \ref{thm_htilde}, proposition \ref{prop_extneg}, lemma \ref{lem_extpos} and  \cite[corollary 3.3.10.b2]{KumBook}.
\qed \\

\begin{prop} \label{prop_h2kac}
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ or in $\Owg_{\Lambda^0}$, with $\Lambda, \Lambda^0 \neq 0$. \\
The following holds:
$$ \text H^{\, 2}(\tglie,M) \ \simeq \ \text{Ext}^{\, 1}_{\glie} (S^+,M) \, . $$
\end{prop}

\proof
Theorem \ref{thm_htilde}, theorem \ref{thm_ext0S}, propositions \ref{prop_extneg} and \ref{prop_Sint} imply:
$$ \text H^2(\tglie,M) \ \simeq \ \text H^2(\glie,M) \, \oplus \, \text{Ext}^1_{\glie} (S^+,M) \, . $$
In another hand, since $M \neq \KK$, one has $\text H^2(\glie,M) = 0$. See \cite[corollary 3.3.10.b3]{KumBook}.
\qed \\

\begin{thm} \label{thm_h2}
Suppose that $\glie$ is finite-dimensional. \\
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ with $\Lambda \neq 0$. The following holds:
$$ \text H^{\, 2}(\tglie,M) \ = \ 0 \, . $$
\end{thm}

\proof
Consequence of propositions \ref{prop_h2kac} and \ref{prop_extpos}.
\qed \\


\begin{rem} \label{rem_end}
The reader could wonder: when $M$ is a $\glie$-module, can actually $\text H^{\, \bullet}(\tglie,M)$ be different from $\text H^{\, \bullet}(\glie,M)$? \\
The answer is positive and one can find such a module $M$ in the category $\Owg$. For example, corollary \ref{cor_SOcat}, lemma \ref{lem_extpos} and theorem \ref{thm_htilde} imply:
$$ \dim \Big( \text H^{\, 1}(\tglie,S^-) \Big) \ > \ \dim \Big( \text H^{\, 1}(\glie,S^-) \Big) \, . $$
Another (however incomplete) example is the following. \\
In view of \cite[proposition 1.5.b]{KumV}, it is possible that $\text H^{\, 2}(\glie,S^-) \neq 0$. In another hand, $\text H^{\, 2}(\glie,S^-) \simeq \text{Ext}^{\, 2}_{\glie}(\KK,S^-) \simeq \text{Ext}^{\, 2}_{\glie}(S^+,\KK)$ (the Cartan involution induces a contravariant equivalence of ${\mathcal O}$ and lemma \ref{lem_SCartan} asserts that $S^+ \simeq (S^-)^{\omega}$). From theorem \ref{thm_htilde}, theorem \ref{thm_ext0S} and corollary \ref{cor_SExt} one then would has:
$$ \dim \Big( \text H^{\, 3}(\tglie) \Big) \ > \ \dim \Big( \text H^{\, 3}(\glie) \Big) \, . $$
\end{rem}



\subsection{Free Serre relations version of second Whitehead's lemma} \label{subs_swhlemma}
Finally, we obtain the free Serre relations version of second Whitehead's lemma, which was the original motivation of this part.

\begin{thm} \label{thm_swhlemma}
Suppose that $\glie$ is finite-dimensional. \\
For all finite-dimensional $\tglie$-modules $M$, one has:
$$ \text H^{\, 2}(\tglie,M) \ = \ 0 \, . $$
\end{thm}

\proof
Recall that $M$ is actually the restriction of a $\glie$-module: see \ref{para_gtildeg}. In view of theorem \ref{thm_h2}, since the category of finite-dimensional $\glie$-modules is completely reducible and since for $\lambda$ dominant, $L(\lambda)$ is in ${\mathcal O}_0$ if and only if $\lambda = 0$, one concludes thanks to theorem \ref{thm_coho2}.
\qed

\begin{rem} \label{rem_fsrvwl1}
A free Serre relations version of first Whitehead's lemma also holds: suppose that $\glie$ is finite-dimensional, then $\text H^{\, 1}(\tglie,M) = 0$ for all finite-dimensional $\tglie$-modules $M$. One can give a proof similar to the proof of theorem \ref{thm_swhlemma}. However this fact is quite straightforward from remark \ref{rem_coho1} and from first Whitehead's lemma. %Actually one can give a even more simpler proof. Let us explain how. \\
%Any $\tglie$-module, extension of two finite-dimensional $\glie$-modules, is integrable since the two latter are. Thus the extension is actually a $\glie$-%module: see \ref{para_gtildeg}. One concludes thanks to first Whitehead's lemma and the following fact (see \cite{Wei}):
%$$ \text H^{\, \bullet} (\alie,N) \ \simeq \ \text{Ext}_{\glie}^{\, \bullet}(\KK,N) \quad \ \text{($\alie$ is a Lie algebra, M,N are $\alie$-modules)} \, . $$
\end{rem}



\subsection{Further} \label{subs_further}
We do not assume here, unless explicitly stated, that $\glie$ is finite-dimensional. We give some consequences of the previous results in order to introduce some open (as far as the author knows) questions and conjectures.

\subsubsection{} \label{para_equivvkac}
We establish precise equivalences between the vanishing of $\text H^{\bullet}(\tglie,M)$ and the vanishing of $\text{Ext}_{\glie}^{\bullet}(S^+,M)$, $\text{Ext}_{\glie}^{\bullet}(S,M)$, when $M$ is in the category ${\mathcal O}$, outside the principal blocks.

\begin{prop} \label{prop_equivkac}
Let $M$ be a $\glie$-module in ${\mathcal O}^{\text g}_{\Lambda}$ or in $\Owg_{\Lambda^0}$ with $\Lambda, \Lambda^0 \neq 0$. \\
For all $n \in \NN$, the following holds:
\begin{multline*}
\Bigg[ \text{Ext}^{\, m-1}_{\glie} (S^+,M) \ = \ \text{Ext}^{\, m-2}_{\glie} (S,M) \ = \ 0 \, , \ \ \forall \ 0 \leq m \leq n \Bigg] \\
\Leftrightarrow \quad \Bigg[ \text H^{\, m}(\tglie,M) \ = \ 0 \, , \ \ \forall \ 0 \leq m \leq n \Bigg] \, . \quad \quad
\end{multline*}
\end{prop}

\proof
Consequence of theorem \ref{thm_htilde}, of proposition \ref{prop_extneg} and the fact that $\text H^{\bullet}(\glie,M)$ vanishes (see \cite[corollary 3.3.10.b2]{KumBook}).
\qed

\begin{cor}
Let $M$ be a $\glie$-module in ${\mathcal O}^{\text g}_{\Lambda}$ or in $\Owg_{\Lambda^0}$ with $\Lambda, \Lambda^0 \neq 0$. \\
The following holds:
$$ \text{Ext}^{\, \bullet}_{\glie} (S^+,M) \ = \ \text{Ext}^{\, \bullet}_{\glie} (S,M) \ = \ 0 \ \quad \Leftrightarrow \quad \ \text H^{\, \bullet}(\tglie,M) \ = \ 0 \, . $$
\end{cor}


\subsubsection{} \label{para_equivvf}
We rewrite previous vanishing equivalences, when $\glie$ is finite-dimensional: in this case, we know that $\text{Ext}^{\bullet}(S^+,M) = 0$ (thanks to the separation of the Weyl orbits by the center of $U(\glie)$, see proposition \ref{prop_extpos}).

\begin{prop}
Suppose that $\glie$ is finite-dimensional. \\
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ with $\Lambda \neq 0$. For all $n \in \NN$, the following holds:
\begin{multline*}
\Bigg[ \text{Ext}^{\, m-2}_{\glie} (S,M) \ = \ 0 \, , \ \ \forall \ 0 \leq m \leq n \Bigg] \\
\Leftrightarrow \quad \Bigg[ \text H^{\, m}(\tglie,M) \ = \ 0 \, , \ \ \forall \ 0 \leq m \leq n \Bigg] \, . \quad \quad
\end{multline*}
\end{prop}

\proof
Consequence of proposition \ref{prop_equivkac} and \ref{prop_extpos}.
\qed

\begin{cor}
Suppose that $\glie$ is finite-dimensional. \\
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ with $\Lambda \neq 0$. The following holds:
$$ \text{Ext}^{\, \bullet}_{\glie} (S,M) \ = \ 0 \ \quad \Leftrightarrow \quad \ \text H^{\, \bullet}(\tglie,M) \ = \ 0 \, . $$
\end{cor}


\subsubsection{}
Some natural conjectures arise. First, proposition \ref{prop_extpos} and lemma \ref{lem_extpos} justifies the following conjecture.

\begin{conj} \label{conj_extpos}
Let $\glie$ be infinite-dimensional and let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ or in $\Owg_{\Lambda^0}$ with $\Lambda, \Lambda^0 \neq 0$. The following holds:
$$ \text{Ext}^{\, \bullet}_{\glie} (S^+,M) \ = \ 0 \, . $$
\end{conj}

Thanks to proposition \ref{prop_h2kac}, conjecture \ref{conj_extpos} implies the following conjecture, which is justified by theorems \ref{thm_h1kac} and \ref{thm_h2}.

\begin{conj} \label{conj_h2kac}
Let $\glie$ be infinite-dimensional and let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ or in $\Owg_{\Lambda^0}$ with $\Lambda, \Lambda^0 \neq 0$. The following holds:
$$ \text H^{\, 2}(\tglie,M) \ = \ 0 \, . $$
\end{conj}


\subsubsection{}
Some natural questions also arise. First, in view of theorem \ref{thm_h1kac}, theorem \ref{thm_h2}, proposition \ref{prop_h2kac}, conjecture \ref{conj_h2kac} and the resemblance with the situation of $\glie$ (recall that $\text H^{\bullet}(\glie,M)$ vanishes: see \cite[corollary 3.3.10.b2]{KumBook}), one is leaded to the following question.

\begin{quest} \label{quest_principalblock}
Let $M$ be a $\glie$-module in ${\mathcal O}_{\Lambda}$ with $\Lambda \neq 0$. \\
Does the following holds:
$$ \text H^{\, \bullet} (\tglie,M) \ = \ 0 \, ? $$
\end{quest}

Finally, in view of the previous results in \ref{para_equivvkac} and \ref{para_equivvf}, and thanks also to conjecture \ref{conj_extpos} in the infinite-dimensional case, it appears that questions \ref{quest_principalblock} is closely related to the following question \ref{quest_extS}.

\begin{quest} \label{quest_extS}
Do $\text{Ext}^{\, \bullet}_{\glie}(S,M)$ and $\text{Ext}^{\, \bullet}_{\glie}(M,S)$ vanish for all $M$ in ${\mathcal O}$?
\end{quest}

Recall that theorem \ref{thm_ext0S} asserts that $\text{Ext}^0_{\glie}(S,M)$ and $\text{Ext}^0_{\glie}(M,S)$ vanish, for all $M$ in ${\mathcal O}$.


\subsubsection{}
As we have understood, cohomology of $\glie$ and $\tglie$ with coefficients in a $\glie$-module are related in terms of some Ext groups of the Serre modules $\glie$-modules $S^{\pm}$ and $S$. Thus, information about these Serre Ext groups give information about cohomology: it was the strategy used in this work to prove among others the free Serre relations version of second Whitehead's lemma. But one can think about the reverse direction. For example, one can obtain the vanishing $\text{Ext}_{\glie}^0(S,\KK)$ from the equality between the second cohomology groups of $\glie$ and $\tglie$ (recall the second proof of theorem \ref{thm_coho2} does not use theorem \ref{thm_ext0S}). Recall also the exceptional cases of theorem \ref{thm_ext0S} were handled thanks to information about cohomologies. \\

This correspondence between cohomology of $\tglie$ and the Serre Ext groups was partly made more precise in \ref{para_equivvkac} and \ref{para_equivvf}. The author ignores which one of the two sides of the correspondence is the easiest to deal with. However, he believes they can be fruitfully combined to get new results about each of them.





\section{Appendices} \label{sect_appendix}
We state and prove here several technical results more or less related to the Serre modules $S^-$, $S^+$ and $S$ (see section \ref{sect_Serre}). They essentially serve the only theorem \ref{thm_ext0S}. \\

The appendix is divided into four parts, each designated by the topic they go into.
\begin{enumerate}
\item[\textbullet] \ref{app_tensor} : Tensor Serre module. \\
We provide the main technical arguments which allow one to establish theorem \ref{thm_ext0S} for the most part. Note this part is sufficient to prove the free Serre relations version of second Whitehead's lemma (theorem \ref{thm_swhlemma}). More precisely, proposition \ref{prop_STHom} asserts that $\text{Ext}^0_{\blie^-}(\KK_{\lambda},S)$ and $\text{Ext}^0_{\blie^-}(S,\KK_{\lambda})$ vanish for all $\lambda \in \hlie^{\ast}$, with however some exceptions in the latter case. \\
The rest of the appendix is essentially devoted to give some other technical arguments used for the remaining exceptional cases of theorem \ref{thm_ext0S}.
\item[\textbullet] \ref{app_npSerre} : Negative and positive Serre modules. \\
There are two main results here. We first that $\text{Ext}^0_{\glie}(S^{\pm},\KK)$ and $\text{Ext}^1_{\glie}(S^{\pm},\KK)$ vanish, this result will be used in the first proof of theorem \ref{thm_coho2}. We also prove that $\text{Ext}^0_{\glie}(S^-,M)$ and $\text{Ext}^1_{\glie}(S^+,M)$ vanishes when $M$ is one the exceptions of proposition \ref{prop_STHom}.
\item[\textbullet]  \ref{app_ext} : Yoneda first extension groups. \\
We prove that for some particular $\glie$-modules $M$, the Yoneda extension groups $\text{YExt}^1_{\glie}(\glie, M)$ and $\text{YExt}^1_{\glie'}(\glie', M)$ are naturally isomorphic, where $\glie'$ designates the quotient of $\glie$ by either the negative, positive or all the Serre relations. Thanks to a classical result (see \cite[theorem 7.6.3]{Wei}), it implies that $\text H^2(\glie, M)$ and $\text H^2(\glie', M)$ are also isomorphic. This result is used in theorem \ref{thm_ext0S} when dealing with the exceptional cases, it is also used in the second proof of theorem \ref{thm_coho2}.
\item[\textbullet] \ref{app_combi} : Combinatorics of the root lattice. \\
We prove some combinatorics results in the root lattice, mostly related to the exceptions which appeared in the statement of proposition \ref{prop_STHom}. Note that lemma \ref{lem_dominant} is only used in the fast way to the free Serre relations version of second Whitehead's lemma.
\end{enumerate}

\begin{remT}
If one is only interested in the proof of theorem \ref{thm_swhlemma}, only proposition \ref{prop_STHom}, proposition \ref{prop_gleqdimext} and its corollary \ref{cor_gleqdimext} are necessary.
\end{remT}

In this section, $\glie$ designates an arbitrary (not necessarily symmetrizable) Kac-Moody algebra (we assume the characteristic of $\KK$ is zero).



\subsection{Tensor Serre module} \label{app_tensor}
The results here are used to establish, for the most part (which is sufficient for the free Serre versions of second Whitehead's lemma), of theorem \ref{thm_ext0S}. \\

Let $\lambda \in \hlie^{\ast}$. By canonically identifying $\text{End}_{\KK}(\KK)$ with $\KK$, $\lambda$ gives rise to a structure of $\hlie$-module on $\KK$. In another hand, $\nlie^-$ is a Lie ideal of the negative Borel subalgebra $\blie^-:= \hlie \oplus \nlie^-$. Thus one has a natural surjective morphism of Lie algebra $\blie^- \to \hlie$. We denote by $\KK_{\lambda}$ the one-dimensional $(\blie^-)$-module obtained by restriction of the $\hlie$-module structure on $\KK$ previously defined from $\lambda$. \\

\begin{prop} \label{prop_STHom}
Let $\lambda \in \hlie^{\ast}$ and denote:
$$ A \ := \Big \{ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, ; \ \ i,j,k,l \in I, \ i \neq j, \, k \neq l \Big \} \, . $$
The following holds:
\begin{enumerate}
\item[1)] $\text{Ext}^{\, 0}_{\blie^-}(\KK_{\lambda},S) = 0 \, ;$
\item[2)] if $\lambda \notin A$, then $\text{Ext}^{\, 0}_{\blie^-}(S,\KK_{\lambda}) \ = \ 0 \, .$
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item[1)] Suppose there is a nonzero morphism $f: \KK_{\lambda} \to S$ of $(\blie^-)$-module. In particular there exists a nonzero vector $v \in S$ which is $(\nlie^-)$-invariant. \\
Let $\mathcal B$ be a linear basis of $S^+$. Then one has:
\begin{equation} \label{eq_MXQ}
S \ = \ \bigoplus_{\mu \in \hlie^{\ast}, \, b \in \mathcal B} \ \Bigg[ S_{\mu}^- \, \otimes_{\KK} \, \Big( \KK . b \Big) \Bigg] \, .
\end{equation}
In particular, there exist $v_{\mu,b} \in S^-_{\mu}$ ($\mu \in \hlie^{\ast}$, $b \in \mathcal B$) such that:
$$ v \ = \ \sum_{\mu \in \hlie^{\ast}, \, b \in \mathcal B} v_{\mu, b} \, \otimes \, b \, , \quad \ K_v \ := \ \Big\{ (\mu,b) \in \hlie^{\ast} \times \mathcal B \, ; \ v_{\mu ,b} \neq 0 \Big\} \ \ \text{ is finite.} $$
Let $\mu'$ a minimal element of $p_1(K_v)$ where $p_1: \hlie^{\ast} \times \mathcal B \to \hlie^{\ast}$ designates the first projection and let $b' \in \mathcal B$ such that $(\mu',b') \in K_v$ (note that $K_v \neq \emptyset$ since $v \neq 0$). \\
Thanks to \eqref{eq_MXQ}, by minimality of $\mu'$ and since $v$ is $(\nlie^-)$-invariant, $v_{\mu',b'}$ is a nonzero vector in $S^-_{\mu'}$ which is $(\nlie^-)$-invariant. \\
Denote $V:= U(\glie) \: \! . \: \! (v_{\mu',b'})$. Since $v_{\mu',b'}$ is $(\nlie^-)$-invariant, $V = U(\nlie^+) \: \! . \: \! (v_{\mu',b'})$ and $\wt V \subset D^{\geq}(\mu')$. From point 3 of lemma \ref{lem_negSerre}, one deduces that $V$ is integrable. From corollary \ref{cor_SOcat}, it follows that $V$ is in ${\mathcal O^{\mathrm{int}}}$. \\
We want to prove that $S^-$ cannot have a submodule in ${\mathcal O^{\mathrm{int}}}$. Since ${\mathcal O^{\mathrm{int}}}$ is completely reducible, one can without loss of generality suppose that $V$ is simple. Moreover, since $V$ is a submodule of $S^-$, there exist $\nu \in \hlie^{\ast}$ and $i, j \in I$ with $i \neq j$ such that $V = L(\nu)$ and such that $\nu \leq - \alpha_j - (1 - a_{ij}) \alpha_i$. Since $V$ is integrable, $\nu$ has to be dominant. It is impossible since:
$$ \alpha_i^{\vee} \Big( - \alpha_j - (1 - a_{ij}) \alpha_i \Big) \ = \ a_{ij} - 2 \ \leq \ -2 \, . $$
We thus have proved that $\text{Ext}^{\, 0}_{\blie^-}(\KK_{\lambda},M) = 0$.
\item[2)] Suppose that $\lambda \notin A$ and that there exists a nonzero morphism $f: M \to \KK_{\lambda}$ of $(\blie^-)$-module. \\
Let $\mu \in \wt (S^-)$ maximal (such a element exists thanks to point 3 of lemma \ref{lem_negSerre}) such that the restriction $f_{\mu}$ of $f$ to $S^-_{\mu} \otimes_{\KK} S^+_{\lambda - \mu}$ is nonzero. \\
Lemma \ref{lem_SCartan} and point 3 of lemma \ref{lem_negSerre} imply that:
$$\mu \ \in \ \bigcup_{k,l \in I, \, k \neq l} D \Big( -\alpha_l - (1 - a_{kl}) \alpha_k \Big) \, , $$
$$ \lambda - \mu \ \in \ \bigcup_{i,j \in I, \, i \neq j} \, D^{\geq} \Big( \alpha_j + (1 - a_{ij}) \alpha_i \Big) \, . $$
Thus, thanks to the hypothesis on $\lambda$, one has:
\begin{equation} \label{eq_lambdamuD}
\lambda - \mu \ \in \ \bigcup_{i,j \in I, \, i \neq j} \, D^> \Big( \alpha_j + (1 - a_{ij}) \alpha_i \Big) \, .
\end{equation}
Let $i \in I$, $v^- \in S^-_{\mu}$ and $v^+ \in S^+_{\lambda - \mu - \alpha_i}$. By maximality of $\mu$, one has:
\begin{eqnarray*}
0 \ = \ e_i . \Big( f(v^- \otimes v^+) \Big) & = & f \Big( (e_i . v^-) \otimes v^+ \Big) \, + \, f \Big( v^- \otimes (e_i .  v^+) \Big) \\
& = & f \Big( v^- \otimes (e_i .  v^+) \Big) \\
& = & f_{\mu} \Big( v^- \otimes (e_i .  v^+) \Big) \, .
\end{eqnarray*}
In another hand, thanks to point 2 of lemma \ref{lem_negSerre}, one has:
$$ (\nlie^-) \, . \, S^- \ = \ \bigoplus_{\lambda \in B} \, S^-_{\lambda} \, , \quad \ \text{ with } \ B \ := \ \bigcup_{i,j \in I, \, i \neq j} D \Big( - \alpha_j - (1 - a_{ij}) \alpha_i \Big) \, . $$
Thus, thanks to lemma \ref{lem_SCartan} and thanks to \eqref{eq_lambdamuD}, it follows that $f_{\mu}$ is zero. This is a contradiction.
\end{enumerate}
\qed



\subsection{Negative and positive Serre modules} \label{app_npSerre}
The results here which are precisely used in this work are the parts ``$\text{Ext}_{\glie}(S^{\pm},\bullet)$" of corollary \ref{cor_SExt} and of point 3 of lemma \ref{lem_extSA}.

\begin{lem} \label{lem_SExt}
Let $M$ be a $\glie$-module such that:
\begin{equation} \label{eq_Dijk}
\wt (M) \, \cap \, D \Big( - \alpha_j + \alpha_k - (1 - a_{ij}) \alpha_i \Big) \ = \ \emptyset \, , \quad \ \forall \, i,j,k \in I, \ i \neq j \, .
\end{equation}
The following holds:
\begin{enumerate}
\item[1)] $\text{Ext}^{\, 0}_{\glie}(S^-,M) \ = \ \text{Ext}^{\, 0}_{\glie}(M,S^-) \ = \ 0 \, ;$
\item[2)] $\text{Ext}^{\, 1}_{\glie}(S^-,M) \ = \ \text{Ext}^{\, 1}_{\glie}(M,S^-) \ = \ 0 \, .$
\end{enumerate}
\end{lem}

\proof
\begin{enumerate}
\item[1)] In view of point 3 of lemma \ref{lem_negSerre}, hypothesis \eqref{eq_Dijk} implies that $\text{wt} \, (S^-) \cap \wt (M) = \emptyset$. One directly deduces:
$$ \text{Hom}_{\glie}(S^-,M) \ = \ \text{Hom}_{\glie}(M,S^-) \ = \ 0 \, . $$
\item[2)] Let $E$ be an extension of $S^-$ by $M$:
$$ \xymatrix{
0 \ar[r] & M \ar[r] & E \ar[r]^p & S^- \ar[r] & 0 \, .
}$$
Thanks to point 5 of lemma \ref{lem_trigonalizable}, $E$ is $\mathfrak h$-trigonalizable. Denote:
$$ E^-:= \bigoplus_{\lambda \in \wt \! (S^-)} E^{\infty}_{\lambda} \, . $$
Point 3 of lemma \ref{lem_negSerre} and hypothesis \eqref{eq_Dijk} imply that $E^-$ is stable under the action of $e_k$, $f_k$ ($k \in I$). Thus $E^-$ is a $\glie$-submodule of $E$. \\
Thanks again to \eqref{eq_Dijk}, one has:
$$ E^- \cap M \ = \ \bigoplus_{\lambda \in \wt \! (S^-)} M^{\infty}_{\lambda} \ = \ 0 \, . $$
As a consequence, the restriction of $p$ to $E^-$ is injective and then an isomorphism of $\glie$-module. It follows that $p$ has a section, i.e. $E$ splits.\\
We have proved that $\text{Ext}^1_{\glie}(S^-,M) = 0$. \\
The proof of $\text{Ext}^1_{\glie}(M,S^-) = 0$ is similar.
\end{enumerate}
\qed \\

\begin{cor} \label{cor_SExt}
The following holds ($\KK$ is seen as a trivial $\glie$-module):
\begin{enumerate}
\item[1)] $\text{Ext}^{\, 0}_{\glie}(S^{\pm},\KK) \ = \ \text{Ext}^{\, 0}_{\glie}(\KK,S^{\pm}) \ = \ 0 \, ;$
\item[2)] $\text{Ext}^{\, 1}_{\glie}(S^{\pm},\KK) \ = \ \text{Ext}^{\, 1}_{\glie}(\KK,S^{\pm}) \ = \ 0 \, .$
\end{enumerate}
\end{cor}

\proof
For $S^-$, it is a consequence of lemma \ref{lem_AD0}. For $S^+$, use the Cartan symmetry \ref{lem_SCartan}.
\qed \\

\begin{lem} \label{lem_extSA}
Denote:
$$ A \ := \ \Big \{ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, ; \ \ i,j,k,l \in I, \ i \neq j, \, k \neq l \Big \} \, . $$
Let $M$ be the simple $\glie$-module $L(\lambda)$, with $\lambda \in A$. The following holds:
\begin{enumerate}
\item[1)] $\text{Ext}^{\, 0}_{\glie}(S^-,M) \ = \ 0 \, ;$
\item[2)] $\text{Ext}^{\, 0}_{\glie}(M,S^+) \ = \ 0 \, ;$
\item[3)] $\text{Ext}^{\, 1}_{\glie}(S^+,M) \ = \ \text{Ext}^{\, 1}_{\glie}(M,S^+) \ = \ 0 \, .$
\end{enumerate}
\end{lem}

\proof
\begin{enumerate}
\item[1)] Suppose there exists a nonzero morphism from $S^-$ to $M$. Denote $\mu_{ij}^- := - \alpha_j - (1 - a_{ij}) \alpha_i$. \\
In view of point 2 of lemma \ref{lem_negSerre}, there exist $i,j \in I$ with $i \neq j$ and a nonzero morphism from $M(\mu_{ij}^-)$ to $M$. This imply that $L(\mu_{ij}^-)$ is isomorphic to $M$ since $M$ is simple. Thus $\mu_{ij}^- = \lambda$, which is impossible in view of \eqref{eq_AD}.
\item[2 \& 3)] Consequence of Cartan symmetry \ref{lem_SCartan}, of lemma \ref{lem_SExt} and of \eqref{eq_ADg}.
\end{enumerate}
\qed

\begin{remmm}
Recall we proved in lemma \ref{lem_extpos} that $\text{Ext}^{\, 0}_{\glie}(S^+,M)$ vanishes for all $M$ in the category ${\mathcal O}$.
\end{remmm}



\subsection{Yoneda first extension groups} \label{app_ext}
The results here are used in the proof of the exceptional cases (which are not needed to establish the free Serre relations of second Whitehead's lemma) of theorem \ref{thm_ext0S}. They are also used in the second proof (which, this time, is needed to established the free Serre relations of second Whitehead's lemma) of theorem \ref{thm_coho2}. \\

\begin{prop} \label{prop_gleqdimext}
Let $M$ be a $\glie$-module.
\begin{enumerate}
\item[1)] If, for all $i,j,k \in I$ with $i \neq j$,
\begin{equation} \label{eq_gleq1}
\wt (M) \ \cap \ D \Big( - \alpha_j + \alpha_k - (1 - a_{ij}) \alpha_i \Big) \ = \ \emptyset \, ,
\end{equation}
then there exists a natural linear isomorphism:
$$ \text{YExt}_{\tglie^-}^{\, 1}(\tglie^-,M) \ \toiso \ \text{YExt}_{\glie}^{\, 1}(\glie,M) \, , \quad \text{where: $\tglie^- := \tglie / \slie^-$} \, . $$
\item[2)] If, for all $i,j,k \in I$ with $i \neq j$,
\begin{equation} \label{eq_gleq2}
\wt (M) \ \cap \ D^{\geq} \Big( \alpha_j - \alpha_k + (1 - a_{ij}) \alpha_i \Big) \ = \ \emptyset \, ,
\end{equation}
then there exists a natural linear isomorphism:
$$ \text{YExt}_{\tglie^+}^{\, 1}(\tglie^+,M) \ \toiso \ \text{YExt}_{\glie}^{\, 1}(\glie,M) \, , \quad \text{where: $\tglie^+ := \tglie / \slie^+$} \, . $$
\item[3)] If, for all $i,j,k \in I$ with $i \neq j$, \eqref{eq_gleq1} and \eqref{eq_gleq2} hold, then there exists a natural linear isomorphism:
$$ \text{YExt}_{\tglie}^{\, 1}(\tglie,M) \ \toiso \ \text{YExt}_{\glie}^{\, 1}(\glie,M) \, . $$
\end{enumerate}
\end{prop}

\proof
We prove point 3. The first two points can be handled in a very analog way. \\

Let $\tilde E$ be a $\tglie$-module, extension of $\tglie$ by $M$:
$$ \xymatrix{
0 \ar[r] & M \ar[r]^{\tilde i} & \tilde E \ar[r]^{\tilde p} & \tglie \ar[r] & 0 \, .
} $$
Thanks to point 5 of lemma \ref{lem_trigonalizable}, $\tilde E$ is $\hlie$-trigonalizable. \\
Denote:
$$ \tilde E^{\pm}_{\slie} \ := \ \left( \bigoplus_{\lambda \in \wt (\tslie^{\pm})} \tilde E^{\infty}_{\lambda} \right) \cap \, \tilde p^{-1} (\tslie^{\pm})  \, , $$
$$ \tilde E_{\slie} \ := \ \tilde E^-_{\slie} \oplus \tilde E^+_{\slie} \, , \quad \quad E \ := \ \tilde E / \tilde E_{\slie} \, . $$
Denote by $\text{pr}_E: \tilde E \to E$ the linear projection naturally associated. \\
Since $\wt (M) \cap \Big( \wt (\tslie^{\pm}) \mp \alpha_k \Big) = \emptyset$ for all $k \in I$, $\tilde E^{\pm}_{\slie}$ is stable under the action of $e_k$ and $f_k$ for all $k \in I$. Thus $\tilde E_{\slie}$ is a $\tglie$-submodule of $\tilde E$. \\
In another hand, since $\wt (M) \cap \wt (\tslie) = \emptyset$, $\tilde i (M) \cap \tilde E_{\slie} = 0$. It follows that the morphism $i:= (\text{pr}_E \circ \tilde i): M \to E$ of $\tglie$-module is injective. \\
Denote by $p: E \to \glie = \tglie / \tslie$ the morphism of $\tglie$-module induced by $\tilde p$. Since $\tilde p$ is surjective, $p$ is also surjective. \\
In conclusion, $E$ is a $\tglie$-module, extension of $\glie$ by $M$ such that $(\text{id}_M, \text{pr}_E, \prg)$ is a morphism of extension from $\tilde E$ to $E$. \\

Let $F$ be a $\tglie$-module, extension of $\glie$ by $M$:
$$ \xymatrix{
0 \ar[r] & M \ar[r]^j & F \ar[r]^q & \glie \ar[r] & 0 \, .
} $$
Let $(\text{id}_M, f, \text{pr}_{\glie})$ be a morphism of extension from $\tilde E$ to $F$. \\
Recall that it means the following diagram commutes:
\begin{equation} \label{eq_extinduced} \xymatrix{
0 \ar[r] & M \ar@{=}[d] \ar[r]^{\tilde i} & \tilde E \ar[r]^{\tilde p} \ar[d]^f & \tglie \ar[r] \ar[d]^{\text{pr}_{\glie}} & 0 \ \, \\
0 \ar[r] & M \ar[r]^j & F \ar[r]^q & \glie \ar[r] & 0 \, .
} \end{equation}
Note that, since $\text{pr}_{\glie}$ is surjective, $f$ is also surjective. \\
Let $\lambda \in \hlie^{\ast}$. The commutativity of \eqref{eq_extinduced} induces, in the category of vector spaces, that the following diagram with exact lines commutes:
\begin{equation} \label{eq_extinduced2} \xymatrix{
0 \ar[r] & M_{\lambda} \ar@{=}[d] \ar[r]^{\tilde i_{\lambda}} & \tilde E_{\lambda} \ar[r]^{\tilde p_{\lambda}} \ar[d]^{f_{\lambda}} & \tglie_{\lambda} \ar[r] \ar[d]^{\text{pr}_{\lambda}} & 0 \ \, \\
0 \ar[r] & M_{\lambda} \ar[r]^{j_{\lambda}} & F_{\lambda} \ar[r]^{q_{\lambda}} & \glie_{\lambda} \ar[r] & 0 \, .
} \end{equation}
If $\lambda \notin \wt (\tslie)$, then $\text{pr}_{\lambda}$ is bijective and thus $f_{\lambda}$ is also bijective. \\
As a consequence, $\ker f$ is contained in $\bigoplus_{\lambda \in \wt \tslie} \tilde E^{\infty}_{\lambda}$. Since $\wt M \cap \wt \slie = \emptyset$, it follows that $\ker f = \tilde E_{\slie}$. \\

In conclusion, we have proved that there exists, up to isomorphism, a unique $\tglie$-module $E$, extension of $\glie$ by $M$, which admits a morphism of extension from $\tilde E$ to itself. \\
As a consequence, this implies that one has a well-defined map:
\begin{eqnarray*}
\Phi \,: \text{YExt}^1_{\tglie}(\tglie,M) & \to & \text{YExt}^1_{\tglie} (\glie,M) \\
\tilde E & \mapsto & E \, .
\end{eqnarray*}
It also implies that the composition $\Phi \circ (\text{pr}_{\tglie})^{\ast}$ is the identity application of $\text{YExt}^1_{\tglie} (\glie,M)$. In another hand, by definition of $(\text{pr}_{\tglie})^{\ast}$, $(\text{pr}_{\tglie})^{\ast} \circ \Phi$ is the identity application of $\text{YExt}^1_{\tglie} (\tglie,M)$. \\
The map $(\text{pr}_{\tglie})^{\ast}$ is then bijective. Since it is linear, it is a linear isomorphism. \\
One concludes thanks to lemma \ref{lem_Ytglie}.
\qed

\begin{cor} \label{cor_gleqdimext}
There exists a natural linear isomorphism ($\KK$ is seen as a trivial $\glie$-module or a trivial $\tglie$-module):
$$ \text{YExt}_{\glie}^1(\glie,\KK) \ \toiso \ \text{YExt}_{\tglie}^1(\tglie,\KK) \, . $$
\end{cor}

\proof
See lemma \ref{lem_AD0}.
\qed



\subsection{Combinatorics of the root lattice} \label{app_combi}
We give here combinatorial lemmas about the weight lattice of $\glie$, mostly related to the exceptions which appeared in proposition \ref{prop_STHom}.

\begin{defi} \label{defi_sharp}
Let $\mu = \sum_{i \in I} m_i \: \! \alpha_i \in Q$. \\
Denote by $\sharp(\mu,\pm)$ the number of $i \in I$ such that $\pm \: \! m_i \geq 1$.
\end{defi}

\begin{lem} \label{lem_AD0}
The following holds:
\begin{equation} \label{eq_AD0}
0 \ \notin \ D \Big( - \alpha_j + \alpha_k - (1 - a_{ij}) \alpha_i \Big) \, , \quad \ \forall \, i,j,k \in I, \ i \neq j \, ,
\end{equation}
\begin{equation} \label{eq_AD0g}
0 \ \notin \ D^> \Big( \alpha_j - \alpha_k + (1 - a_{ij}) \alpha_i \Big) \, , \quad \ \forall \, i,j,k \in I, \ i \neq j \, .
\end{equation}
\end{lem}

\proof
Suppose the contrary of \eqref{eq_AD0}, then $\sharp(0,-) \geq 1$ (recall that $a_{ij} \leq 0$), this is a contradiction. \\
Since $0 = -0$, \eqref{eq_AD0g} follows from \eqref{eq_AD0}.
\qed \\

The following combinatorial lemma \ref{lem_AD} is a generalisation of previous lemma \ref{lem_AD0}.

\begin{lem} \label{lem_AD}
Denote:
$$ A \ := \ \Big \{ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, ; \ \ i,j,k,l \in I, \ i \neq j, \, k \neq l \Big \} \, . $$
The following holds:
\begin{equation} \label{eq_AD}
A \, \cap \, D \Big( - \alpha_{j'} + \alpha_{k'} - (1 - a_{i'j'}) \alpha_{i'} \Big) \ = \ \emptyset \, , \quad \ \forall \, i',j',k' \in I, \ i' \neq j' \, ,
\end{equation}
\begin{equation} \label{eq_ADg}
A \, \cap \, D^{\geq} \Big( \alpha_{j'} - \alpha_{k'} + (1 - a_{i'j'}) \alpha_{i'} \Big) \ = \ \emptyset \, , \quad \ \forall \, i',j',k' \in I, \ i' \neq j' \, ,
\end{equation}
\end{lem}

\proof
Remark that, since $-A = A$, \eqref{eq_ADg} is equivalent to \eqref{eq_AD}. Let us prove \eqref{eq_AD}. \\
Suppose there exist $i,j,k,l \in I$ with $i \neq j$, $k \neq l$ and $i', j', k' \in I$ with $i' \neq j'$, such that:
\begin{equation} \label{eq_muijkl}
\mu_{ij}^{kl} \,:= \, \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \ \in \ D \Big( - \alpha_{j'} + \alpha_{k'} - (1 - a_{i'j'}) \alpha_{i'} \Big) \, .
\end{equation}
Let us distinguish two cases.
\begin{enumerate}
\item[1)] $k' \notin \{i',j'\}$. Since $i' \neq j'$, $i'$, $j'$ and $k'$ are pairwise distinct. It implies that $i$, $j$, $k$ and $l$ are pairwise distinct. Let us prove it.
\begin{enumerate}
\item[\textbullet] Thanks to \eqref{eq_muijkl}, $\sharp(\mu_{ij}^{kl},-) \leq 2$. Thus $l \notin \{ i,j \}$.
\item[\textbullet] Suppose that $i = k$.  Thus $k' = j$ and there are two cases.
\begin{enumerate}
\item[a)] $j' = l$ and $i' = k$. Then \eqref{eq_muijkl} implies that:
$$ \alpha_j - \alpha_l - (-a_{kl} + a_{ij}) \alpha_k \ \leq \ \alpha_j - \alpha_l - (1 -a_{kl}) \alpha_k \, . $$
This is a contradiction since $a_{ij} \leq 0$.
\item[b)] $j' = k$ and $i' = l$.  Hypothesis \eqref{eq_muijkl} implies that:
\begin{equation} \label{eq_mujlk}
\alpha_j - \alpha_l - (-a_{kl} + a_{ij}) \alpha_k \ \leq \ \alpha_j - (1 - a_{lk}) \alpha_l - \alpha_k \, .
\end{equation}
Since $k \neq l$, it follows that $a_{lk} = 0$. Thus $a_{kl} = 0$ and \eqref{eq_mujlk} then implies that $a_{ij} \geq 1$. This is a contradiction.
\end{enumerate}
\item[\textbullet] Suppose that $j = k$. Thus $k' = i$, $a_{ij} = 0$ and there are two cases.
\begin{enumerate}
\item[a)] $j' = l$ and $i' = k$. Then \eqref{eq_muijkl} implies that:
$$ - \alpha_l + \alpha_i + a_{kl} \, \alpha_k \ \leq \ - \alpha_l + \alpha_i - (1 -a_{kl}) \alpha_k \, . $$
This is a contradiction.
\item[b)] $j' = k$ and $i' = l$.  Hypothesis \eqref{eq_muijkl} implies that:
$$ - \alpha_l + \alpha_i + a_{kl} \, \alpha_k \ \leq \ - (1 - a_{lk}) \alpha_l + \alpha_i - \alpha_k \, . $$
Since $k \neq l$, it follows that $a_{kl} <  0$ and that $a_{lk} \geq 0$. This a contradiction.
\end{enumerate}
\end{enumerate}
As a consequence, $\sharp(\mu_{ij}^{kl},+) \geq 2$. But, thanks to \eqref{eq_muijkl}, $\sharp(\mu_{ij}^{kl},+) \leq 1$. This is a contradiction.
\item[2)] $k' \in \{i',j'\}$. Thanks to \eqref{eq_muijkl}, $\sharp(\mu_{ij}^{kl},+) = 0$ and $\sharp(\mu_{ij}^{kl},-) \geq 1$. \\
$\sharp(\mu_{ij}^{kl},+) = 0$ implies that $\{ k,l \} = \{ i,j \}$. There are three cases.
\begin{enumerate}
\item[a)] $i = k$ and $j = l$. $\mu_{ij}^{kl} = 0$, then $\sharp(\mu_{ij}^{kl},-) = 0$. This is a contradiction.
\item[b)] $i = l$, $j = k$ and $a_{il} = a_{ji} = 0$. $\mu_{ij}^{kl} = a_{ji} \: \! \alpha_j - a_{ij} \alpha_i = 0$, then $\sharp(\mu_{ij}^{kl},-) = 0$. This is a contradiction.
\item[c)] $i = l$, $j = k$ and $a_{ij} < 0$. $\mu_{ij}^{kl} = a_{ji} \: \! \alpha_j - a_{ij} \alpha_i$, thus $\sharp(\mu_{ij}^{kl},+) \geq 1$. This is a contradiction.
\end{enumerate}
\end{enumerate}
\qed \\

The following lemma \ref{lem_dominant} is only used in the fast way to theorem \ref{thm_swhlemma}. See the ``Towards" remark which follows theorem \ref{thm_ext0S}.

\begin{lem} \label{lem_dominant}
Denote:
$$ A \ := \ \Big \{ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, ; \ \ i,j,k,l \in I, \ i \neq j, \, k \neq l \Big \} \, . $$
The only dominant weight of $A$ is $0$.
\end{lem}

\proof
Denote: $\lambda:= \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k$ and suppose that $\lambda \neq 0$. \\
One can then distinguish 4 cases.
\begin{enumerate}
\item[1)] $k$ is distinct from $i$ and $j$. One has:
\begin{eqnarray*}
\lambda(\alpha_k^{\vee}) & = & a_{kj} - a_{kl} + (1 - a_{ij}) \: \! a_{ki} - 2 \: \! (1 - a_{kl}) \\
& = & a_{kj} + a_{kl} + (1 - a_{ij}) \: \! a_{ki} - 2 \\
& \leq & -2 \, .
\end{eqnarray*}
The last inequality follows from the fact that $k$ is distinct from $i$, $j$ and $l$. Thus $\lambda$ is not dominant.
\item[2)] $k = i$, $l \neq j$ and $a_{il} \geq a_{ij}$. One has:
\begin{eqnarray*}
\lambda(\alpha_l^{\vee}) & = & a_{lj} - 2 + (1 - a_{ij}) \: \! a_{li} - (1 - a_{il}) \: \! a_{li} \\
& = & a_{lj} + (a_{il} - a_{ij}) \: \! a_{li} - 2 \\
& \leq & -2 \, .
\end{eqnarray*}
The last inequality follows from the fact that $l$ is distinct from $i$ and $j$. Thus $\lambda$ is not dominant.
\item[3)] $k = i$, $l \neq j$ and $a_{il} < a_{ij}$. One has:
\begin{eqnarray*}
\lambda(\alpha_i^{\vee}) & = & a_{ij} - a_{il} + 2 \: \! (1 - a_{ij}) - 2 \: \! (1 - a_{il}) \\
& = & - a_{ij} + (a_{il} \, . \\
& \leq & -2 \, .
\end{eqnarray*}
Thus $\lambda$ is not dominant.
\item[4)] $k = j$, $l \neq i$; either $a_{ij} < 0$ or $a_{jl} < 0$. One has:
\begin{eqnarray*}
\lambda(\alpha_j^{\vee}) & = & 2 - a_{jl} + (1 - a_{ij}) \: \! a_{ji} - 2 \: \! (1 - a_{jl}) \\
& = & a_{jl} + (1 - a_{ij}) \: \! a_{ji} \, .
\end{eqnarray*}
Thus $\lambda$ is not dominant (recall that $a_{ij} < 0$ if and only if $a_{ji} < 0$).
\item[5)] $k = j$, $l \neq i$ and $a_{ij} = a_{jl}$. One has (recall that $a_{lj} = a_{jl} = 0$):
\begin{eqnarray*}
\lambda(\alpha_l^{\vee}) & = & a_{lj} - 2 + (1 - a_{ij}) \: \! a_{li} - (1 - a_{jl}) \: \! a_{lj} \\
& = & a_{li} - 2 \\
& \leq & -2 \, .
\end{eqnarray*}
The last inequality follows from the fact that $l$ is distinct from $i$. Thus $\lambda$ is not dominant.
\end{enumerate}
\qed \\

\begin{remmm}
When $\glie$ is finite-dimensional, lemma \ref{lem_dominant} is a direct consequence of a more general fact. \\
Let $A$ be the Cartan matrix of $\glie$. We adopt the following notation: for a integral column vector $u = {}^t (u_1, \dots, u_l)$, we write $u > 0$ and $u \geq 0$ if respectively $u_k > 0$ and $u_k \geq 0$ for all $k$. It is known (see \cite[theorem 4.3]{Kac}) that if $A$ is of finite type, then $A \: \! u \geq 0$ implies $u > 0$ or $u = 0$. \\
Let $i,j,k,l \in I$ with $i \neq j$ and $k \neq l$ and define a column vector $u$ by:
$$ \sum_{s \in I} \, u_s \: \! \alpha_s \ = \ \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k \, . $$
$\lambda:= \alpha_j - \alpha_l + (1 - a_{ij}) \alpha_i - (1 - a_{kl}) \alpha_k$ is dominant if and only if $A \: \! u \geq 0$. Thus if $\lambda$ is dominant, then $u > 0$ or $u = 0$. In another hand, in view of the definition of $A$, one cannot have $u > 0$ if $u \neq 0$.
\end{remmm}


==> Nomencl/nomencl.tex <==
\renewcommand{\nomname}{Index des Notations et Définitions}
\renewcommand*{\pagedeclaration}[1]{\hfill \hyperpage{#1}}
\setlength{\nomitemsep}{0cm}
\RequirePackage{ifthen}
\renewcommand{\nomgroup}[1]{%
\ifthenelse{\equal{#1}{A}}{\item[\large{\textbf{I. Generalised Quantum Enveloping Algebras}}] \vspace*{0.2cm} \item[\underline{\textbf{Conventions}}] \vspace*{0.4cm} \item[] \vspace*{-0.4cm}}{%
\ifthenelse{\equal{#1}{B}}{\item[\textbf{1. \textsc{Framework}}] \vspace*{0.5cm} \item[\underline{\textbf{1.1. Kac-Moody algebras}}] \vspace*{0.1cm} \item[] \vspace*{-0.3cm}}{%
\ifthenelse{\equal{#1}{C}}{\item[\dotfill]}{%
\ifthenelse{\equal{#1}{D}}{\item[\underline{\textbf{1.2. Modules and algebras over a power series ring}}] \vspace*{0.5cm} \item[] \vspace*{-0.3cm}}{%
\ifthenelse{\equal{#1}{E}}{\item[\dotfill]}{%
\ifthenelse{\equal{#1}{F}}{\item[\underline{\textbf{1.3. Pointed diagrams of algebras and formal deformations}}] \vspace*{0.5cm} \item[] \vspace*{-0.3cm}}{%
\ifthenelse{\equal{#1}{G}}{\item[\dotfill]}{%
\ifthenelse{\equal{#1}{X}}{\item[\textbf{2. \textsc{GQE Algebras of Rank One}}] \vspace*{0.5cm}}{%
\ifthenelse{\equal{#1}{Y}}{\item[\textbf{3. \textsc{GQE Algebras: General Case}}]}{}}}}}}}}}}

